Online Submodular Maximization via Online Convex Optimization

We study monotone submodular maximization under general matroid constraints in the online setting. We prove that online optimization of a large class of submodular functions, namely, weighted threshold potential functions, reduces to online convex optimization (OCO). This is precisely because functions in this class admit a concave relaxation; as a result, OCO policies, coupled with an appropriate rounding scheme, can be used to achieve sublinear regret in the combinatorial setting. We show that our reduction extends to many different versions of the online learning problem, including the dynamic regret, bandit, and optimistic-learning settings.

==> figs/compare.tex <==

\begin{table*}[!t]
\resizebox{\textwidth}{!}{
\begin{tiny}
\begin{tabular}{||c||c||c|c|c||c|c|c||c|c|c||c||}
\hline
 & \multicolumn{1}{c||}{}  &\multicolumn{9}{c||}{\textbf{$(1-1/e)$-regret (Full Information)}} & \\
\cline{3-11}
\textbf{Paper}  & \textbf{Prob. Class} &\multicolumn{3}{c||}{\textbf{Static}}&\multicolumn{3}{c||}{\textbf{Dynamic}} & \multicolumn{3}{c||}{\textbf{Optimistic}} &  \textbf{Time} \\
\cline{3-11}
&&\textbf{Uni.}&\textbf{Part.}&\textbf{Gen.}&\textbf{Uni.}&\textbf{Part.}&\textbf{Gen.}&\textbf{Uni.}&\textbf{Part.}&\textbf{Gen.}&\\
\hline
\cite{niazadeh2021online} & GS& $r\sqrt{\log\parentheses{n} T}$&\xmark&\xmark&\xmark&\xmark&\xmark&\xmark&\xmark & \xmark & $T^4 O_b$\\
\hline
\cite{harvey2020improved}& GS& \multicolumn{3}{c||}{$ \sqrt{r\log\parentheses{\frac{n}{r}} T}$}&\xmark &\xmark &\xmark&\xmark&\xmark&\xmark&\parbox{2cm}{ \centering $n r^2 + O_{\mathrm m}\cdot n^4/\epsilon^3$ \\ $\textstyle\log({{n^3 T}/{\epsilon}})$ }\\
\hline
\cite{matsuoka2021tracking}  & GS&$r  \sqrt{ r\log(nT) T}$&\xmark&\xmark&$\sqrt{r (r\log(nT) + P_T) T}$&\xmark&\xmark&\xmark & \xmark & \xmark &   ${n r}$\\
\hline
\cite{onlineassignement}  & GS & \multicolumn{2}{c|}{\!\!\!$r^{\frac{3}{2}} \sqrt{ \log(n) T} $ }&\xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  & ${n^2 c_{\mathrm p} }$\\ 
\hline
\hline
% \cite{wan2023bandit}  & GS &\multicolumn{3}{c||}{\xmark}& \multicolumn{2}{c|}{$r^{\frac{4}{3}} n^{\frac{4}{3}}T^{\frac{2}{3}}$}& \xmark & \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $ n r^2$ \\
\cite{chen2018online}  & DR-S&\multicolumn{3}{c||}{$\sqrt{rnT}$}& \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $\sqrt{T} O_{\mathrm {oco}}\cdot O_{\mathrm m}+ n r^2$ \\
\hline
\cite{zhang2019online}  & DR-S&\multicolumn{3}{c||}{$T^{\frac{4}{5}}$ }&  \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $ T^{\frac{3}{5}} O_{\mathrm{oco}}\cdot O_{\mathrm m}+ n r^2 $ \\
\hline
\cite{zhang2022stochastic}  & DR-S&\multicolumn{3}{c||}{$\sqrt{rnT}$ }& \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $O_{\mathrm{oco}} \cdot O_{\mathrm m}+ n r^2 $  \\
\hline
\hline
\cite{kakade2007playing}  & LWD&\multicolumn{3}{c||}{$n(\alpha+2) \sqrt{T}$ }&  \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $ T O_{\mathrm{\alpha}}$ \\
\hline
\hline
\paintbg \parbox{.25cm}{\centering This work}& \parbox{1cm}{\centering\paintbg WTP}& \multicolumn{3}{c||}{\paintbg $r\sqrt{\log(\frac{n}{r}) T}$}  & \multicolumn{3}{c|}{\paintbg $\sqrt{r (r\log(\frac{n}{r}) + \log(n) P_T) T}$}&\multicolumn{3}{c|}{\paintbg \parbox{2.7cm}{\centering $\sqrt{r (r\log(\frac{n}{r}) + \log(n) P_T)}t$\\  $\cdot \sqrt{\displaystyle\sum^T_{t =1} \norm{\g_t - \g_t^\pi}_\infty^2}$} }&\paintbg ${n r^2}$\\
\hline
\end{tabular}
\end{tiny}
}
\caption{Order ($\BigO{\,\cdot\,}$) comparison of regrets and time complexities attained by different online submodular optimization algorithms for general submodular  (GS) and others for continuous DR-submodular  (DR-S) functions. We also include~\citet{kakade2007playing}, who operate on Linearly Weighted Decomposable (LWD) functions, and our work on Weighted Threshold Potential (WTP) functions. 
% The footnote (\textsuperscript{$\dagger$}) indicates that  our algorithm extends to GS class in the bandit setting. 
We also indicate whether algorithms operate over uniform, partition, or general matroid constraints, in the static , bandit, and optimistic settings. Regret and complexity are characterized in terms of the time horizon $T$, the  ground set size $n$, the matroid rank $r$. Additional, algorithm-specific parameters are specified in Appendix~\ref{appendix:additional_related_work}, and the derivation of the regret constants in this work is provided in Appendix~\ref{appendix:setups_omd}.
% : $C$ the size of color palette, $\vec{\mathcal{A}}_b$ is a Blackwell approachability policy,  $\vec{\mathcal{A}}_{\mathrm{FTRL}}$ is an FTRL policy, $\vec{\mathcal{A}}_{\mathrm{OLO}}$ is an online linear optimization policy, and $\vec{\mathcal{A}}_{\mathrm{OGA}}$ is online gradient ascent. %In the full information setting, all algorithms yield $O(\sqrt{T})$ $\alpha$-regret.
The SoTA general submodular+general matroid algorithm \cite{harvey2020improved} has a tighter regret than us by a factor $\sqrt{r}$, but has a much higher computational complexity. We attain the same or or better regret than the DR-S \cite{chen2018online,zhang2019online,zhang2022stochastic}  and remaining algorithms, that also either operate on restricted constraint sets \cite{niazadeh2021online,matsuoka2021tracking, onlineassignement} or on the much more restrictive LWD class \cite{kakade2007playing}.
% In the bandit setting competing algorithms that outperform us either only operate on limited constraint sets \cite{niazadeh2021online,onlineassignement} or the LWD class \cite{kakade2007playing}, while \cite{zhang2019online} attain worse regret; with the exception of the work of~\cite{wan2023bandit} which attains a tighter regret in the static setting over GS class, however when we employ a specialized static OCO algorithm we attain the same bound.
Most importantly, our work readily generalizes to the dynamic and optimistic settings. With the sole exception of \citet{matsuoka2021tracking}, who study dynamic regret restricted to uniform matroids,  our work is the  first to provide guarantees for online submodular optimization in the dynamic and optimistic settings under general matroid constraints. Leveraging the concave relaxation and eschewing computing the multilinear relaxation also yields significant computational complexity dividends. }
% \vspace*{-15pt}
\label{table:compare}
\end{table*}


==> figs/experimental_result_table.tex <==

\begin{table*}[!t]
    \renewcommand{\arraystretch}{1.2}

    \centering
    \resizebox{\textwidth}{!}{%
    % \begin{tiny}
    \begin{tabular}{|c|c|c|c||c|c|c||c|c|c|c||c|c|c|c||c|c|c|c||c|c|}
    \cline{5-21}
         \multicolumn{4}{c}{} & \multicolumn{3}{|c||}{\RAOCOOGA{}} & \multicolumn{4}{c||}{\RAOCOOMA{}} & \multicolumn{4}{c||}{$\texttt{FSF}^\star$} & \multicolumn{4}{c||}{\texttt{TabularGreedy}} & \multicolumn{2}{c|}{\texttt{Random}} \\
    \hline
        \multicolumn{2}{|c|}{\makecell{Datasets \\ \& Constr.}} & $F^\star$ &$t$ & $\bar{F}_{\X}/F^\star$ & std. dev. & $\eta$ & $\bar{F}_{\X}/F^\star$ & std. dev. & $\eta$ & $\gamma$ & $\bar{F}_{\X}/F^\star$ & std. dev. & $\eta$ & $\gamma$ & $\bar{F}_{\X}/F^\star$ & std. dev. & $\eta$ & $c_{\mathrm p}$ & $\bar{F}_{\X}/F^\star$ & std. dev.  \\
    \hline
         \multirow{6}{*}{\rotatebox{90}{\IMZKC}} & \multirow{3}{*}{\rotatebox{90}{uniform}} & \multirow{3}{*}{$0.234$} & $33$ & $0.902$ & $1.85\times 10^{-2}$ & \multirow{3}{*}{$2.5$} & $\mathbf{0.965}$ & $6.02\times 10^{-3}$ & \multirow{3}{*}{$10$} & \multirow{3}{*}{$0.05$} & $0.839$ & $5.02\times 10^{-3}$ & \multirow{3}{*}{$75$} & \multirow{3}{*}{$0.0$} & $0.833$ & $8.12\times 10^{-3}$ & \multirow{3}{*}{$160$} & \multirow{3}{*}{$1$} & $0.642$ & $3.03 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                                                 &                              &                          & $66$ & $0.924$ & $1.60\times 10^{-2}$ &  & $\mathbf{0.967}$ & $5.65\times 10^{-3}$ & & & $0.896$ & $3.83\times 10^{-3}$ &  & & $0.894$ & $2.55\times 10^{-3}$ & & & $0.624$ & $2.80 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                                                 &                              &                         & $99$ & $0.945$ & $7.70\times 10^{-3}$ &  & $\mathbf{0.982}$ & $5.28\times 10^{-3}$ & & & $0.933$ & $4.17\times 10^{-3}$ &  & & $0.931$ & $1.47\times 10^{-3}$ & & & $0.622$ & $1.91 \times 10^{-2}$\\
    \cline{2-21}
                                                 & \multirow{3}{*}{\rotatebox{90}{partition}}                                      & \multirow{3}{*}{$0.83$} & $33$ & $0.994$ & $2.52\times 10^{-3}$ & \multirow{3}{*}{$8$} & $\mathbf{0.997}$ & $6.95\times 10^{-4}$ & \multirow{3}{*}{$10$} & \multirow{3}{*}{$0.1$}  & \multicolumn{4}{c||}{\multirow{3}{*}{\xmark}} & $0.985$ & $5.65\times 10^{-3}$ & \multirow{3}{*}{$10$} & \multirow{3}{*}{$1$}& $0.953$ & $4.88 \times 10^{-3}$\\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                                 & & & $66$ & $0.99$ & $8.75\times 10^{-4}$ &  & $\mathbf{0.994}$ & $3.48\times 10^{-4}$ & & & \multicolumn{4}{c||}{} & $0.987$ & $2.93\times 10^{-3}$ & & & $0.950$ & $2.87 \times 10^{-3}$\\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                                 & & & $99$ & $0.993$ & $9.66\times 10^{-4}$ &  & $\mathbf{0.997}$ & $3.37\times 10^{-4}$ & & &\multicolumn{4}{c||}{}& $0.995$ & $2.70\times 10^{-3}$ & & & $0.953$ & $1.77 \times 10^{-3}$\\
    \hline
         \multirow{6}{*}{\rotatebox{90}{\IMEpinions}} & \multirow{3}{*}{\rotatebox{90}{uniform}} & \multirow{3}{*}{$0.171$} & $50$ & $0.845$ & $1.61\times 10^{-2}$ & \multirow{3}{*}{$4$} & $\mathbf{0.853}$ & $2.46\times 10^{-2}$ & \multirow{3}{*}{$10$} & \multirow{3}{*}{$0.01$} & $0.703$ & $6.03\times 10^{-2}$ & \multirow{3}{*}{$75$} & \multirow{3}{*}{$0.0$} & $0.694$ & $3.44\times 10^{-2}$ & \multirow{3}{*}{$160$} & \multirow{3}{*}{$1$} & $0.632$ & $2.99 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                & & & $100$ & $0.865$ & $1.13\times 10^{-2}$ & & $\mathbf{0.906}$ & $1.25\times 10^{-2}$ & & & $0.776$ & $1.28\times 10^{-2}$ &  & & $0.768$ & $2.87\times 10^{-2}$ & & & $0.615$ & $2.32 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                & & & $149$ & $0.88$ & $7.97\times 10^{-3}$ & & $\mathbf{0.925}$ & $9.09\times 10^{-3}$ & & & $0.807$ & $1.52\times 10^{-2}$ &  & & $0.805$ & $2.48\times 10^{-2}$ & & & $0.629$ & $2.36 \times 10^{-2}$\\
    \cline{2-21}
                & \multirow{3}{*}{\rotatebox{90}{partition}} & \multirow{3}{*}{$0.171$} & $50$ & $0.826$ & $1.35\times 10^{-2}$ & \multirow{3}{*}{$3$} & $\mathbf{0.861}$ & $1.82\times 10^{-2}$ & \multirow{3}{*}{$10$} & \multirow{3}{*}{$0.001$} & \multicolumn{4}{c||}{\multirow{3}{*}{\xmark}} & $0.720$ & $2.28\times 10^{-2}$ & \multirow{3}{*}{$160$} & \multirow{3}{*}{$1$} & $0.620$ & $6.08 \times 10^{-3}$\\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                                 & & & $100$ & $0.854$ & $6.73\times 10^{-3}$ & & $\mathbf{0.908}$ & $9.42\times 10^{-3}$ & & & \multicolumn{4}{c||}{} & $0.786$ & $1.27\times 10^{-2}$ & & & $0.619$ & $4.70 \times 10^{-3}$\\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                                 & & & $149$ & $0.88$ & $2.40\times 10^{-3}$ &  & $\mathbf{0.927}$ & $6.34\times 10^{-3}$ & & & \multicolumn{4}{c||}{} & $0.818$ & $1.3\times 10^{-2}$ & & & $0.625$ & $1.10 \times 10^{-2}$\\
    \hline
         \multirow{6}{*}{\rotatebox{90}{\FLMovieLens{}}} & \multirow{3}{*}{\rotatebox{90}{uniform}} & \multirow{3}{*}{$0.407$} & $98$ & $0.749$ & $3.21\times 10^{-2}$ & \multirow{3}{*}{$0.5$} & $\mathbf{0.792}$ & $2.60\times 10^{-2}$ & \multirow{3}{*}{$1.0$} & \multirow{3}{*}{$0.05$} & $0.681$ & $8.41\times 10^{-2}$ & \multirow{3}{*}{$1.0$} & \multirow{3}{*}{$0.001$} & $0.69$ & $1.11\times 10^{-2}$ & \multirow{3}{*}{$160$} & \multirow{3}{*}{$1$} & $0.748$ & $5.26 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                                 & & & $196$ & $\mathbf{0.786}$ & $3.82\times 10^{-2}$ &  & $0.781$ & $1.36\times 10^{-2}$ & & & $0.713$ & $7.44\times 10^{-2}$ & & & $0.676$ & $1.03\times 10^{-2}$ & & & $0.7$ & $4.76 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                                 & & & $293$ & $0.846$ & $3.98\times 10^{-2}$ &  & $\mathbf{0.866}$ & $1.02\times 10^{-2}$ & & & $0.756$ & $6.42\times 10^{-2}$ &  & & $0.769$ & $1.65\times 10^{-2}$ & & & $0.711$ & $3.11 \times 10^{-2}$\\
    \cline{2-21}
                                 & \multirow{3}{*}{\rotatebox{90}{partition}} & \multirow{3}{*}{$0.419$} & $98$ & $0.889$ & $5.20\times 10^{-2}$ & \multirow{3}{*}{$0.5$} & $\mathbf{0.948}$ & $9.70\times 10^{-3}$ & \multirow{3}{*}{$10$} & \multirow{3}{*}{$0.001$} & \multicolumn{4}{c||}{\multirow{3}{*}{\xmark}} & $0.908$ & $2.39\times 10^{-2}$ & \multirow{3}{*}{$160$} & \multirow{3}{*}{$8$} & $0.829$ & $5.54 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                                 & & & $196$ & $0.872$ & $2.12\times 10^{-2}$ &  & $\mathbf{0.908}$ & $5.14\times 10^{-3}$ & & & \multicolumn{4}{c||}{} & $0.902$ & $1.98\times 10^{-2}$ & & & $0.814$ & $1.51 \times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                                 & & & $293$ & $0.926$ & $2.34\times 10^{-2}$ &  & $0.948$ & $3.13\times 10^{-3}$ & & & \multicolumn{4}{c||}{} & $\mathbf{0.964}$ & $2.01\times 10^{-2}$ & & & $0.874$ & $2.84 \times 10^{-3}$\\
    \hline
         \multirow{6}{*}{\rotatebox{90}{\TeamFormation}} & \multirow{3}{*}{\rotatebox{90}{uniform}} & \multirow{3}{*}{$200$}  & $33$ & $0.984$ & $7.05\times 10^{-3}$ & \multirow{3}{*}{$4$} & $\mathbf{0.987}$ & $4.03 \times 10^{-3}$ & \multirow{3}{*}{$0.05$} & \multirow{3}{*}{$0.1$} & $0.845$ & $4.73 \times 10^{-2}$ & \multirow{3}{*}{$1$} & \multirow{3}{*}{$0$} & $0.844$ & $2.21\times 10^{-2}$ & \multirow{3}{*}{$1$} & \multirow{3}{*}{$2$} & $0.605$ & $3.13\times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                 & & & $66$ & $0.994$ & $3.87 \times 10^{-3}$ &  & $\mathbf{0.994}$ & $2.83 \times 10^{-3}$ & & & $0.868$ & $2.14\times 10^{-2}$ & & & $0.886$ & $1.88\times 10^{-2}$ & & & $0.603$ & $2.01\times 10^{-2}$\\
    \cline{4-6}\cline{8-9}\cline{12-13}\cline{16-17}\cline{20-21}
                 & & & $99$ & $0.995$ & $2.01 \times 10^{-3}$ &  & $\mathbf{0.998}$ & $2.55 \times 10^{-3}$ & & & $0.869$ & $2.95\times 10^{-2}$ & & & $0.902$ & $2.28\times 10^{-2}$ & & & $0.612$ & $1.18\times 10^{-2}$\\
    \cline{2-21}
                 & \multirow{3}{*}{\rotatebox{90}{partition}} & \multirow{3}{*}{$400$} & $33$ & $0.98$ & $3.48 \times 10^{-3}$ & \multirow{3}{*}{$3$} & $\mathbf{0.983}$ & $2.33 \times 10^{-3}$ & \multirow{3}{*}{$0.1$} & \multirow{3}{*}{$0.001$} & \multicolumn{4}{c||}{\multirow{3}{*}{\xmark}} & $0.834$ & $4.01\times 10^{-3}$ & \multirow{3}{*}{$1$} & \multirow{3}{*}{$1$} & $0.611$ & $9.15\times 10^{-3}$\\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                & &  & $66$ & $0.990$ & $1.75 \times 10^{-3}$ &  & $\mathbf{0.991}$ & $1.18 \times 10^{-3}$ & & & \multicolumn{4}{c||}{} & $0.852$ & $2.04\times 10^{-3}$ & & & $0.607$ & $5.44\times 10^{-3}$ \\
    \cline{4-6}\cline{8-9}\cline{16-17}\cline{20-21}
                & &  & $99$ & $0.993$ & $1.11 \times 10^{-3}$ &  & $\mathbf{0.994}$ & $7.75\times 10^{-4}$ & & & \multicolumn{4}{c||}{} & $0.857$ & $1.36\times 10^{-3}$ & & & $0.601$ & $7.71\times 10^{-3}$\\
    \hline
    % \bottomrule
    \end{tabular}       
    % \end{tiny}
    }
    \caption{Average cumulative reward $\bar{F}_{\X}$ ($t = T/3, 2T/3, T$), normalized by fractional optimal $F^\star$, of integral policies across different datasets and constraints. Optimal hyperparameters ($\eta, \gamma, c_{\mathrm p}$) are reported with each algorithm (see Appendix~\ref{sec:experiments} for value ranges explored). \Algorithm{RAOCO} combined with \Algorithm{OGA} or \Algorithm{OMA} outperforms competitors almost reaching one, with the exception of \texttt{MovieLens}, where \Algorithm{TabularGreedy} does better. As \Algorithm{Random} also performs well on \texttt{MovieLens}, this indicates that the (static) offline optimal is quite poor for this reward sequence.   By Property~\ref{assumption:sandwich}, fractional solutions strictly dominate the integral optimal, which implies that in all cases \Algorithm{RAOCO} outperformed the $1-1/e$ approximation, attaining an almost optimal value.  }
 %   \vspace*{-20pt}
    \label{tab:res}
\end{table*}


==> figs/plots.tex <==
\begin{figure}[t]
    \centering
    \subcaptionbox{Stationary}{\includegraphics[height = .21\textwidth,trim={0 0 .5cm 0}]{figs/stationary.pdf}}
    \subcaptionbox{Non-Stationary}{\hspace*{-10pt}\includegraphics[height = .21\textwidth, trim={0.54cm 0 .7cm 0},clip]{figs/dynamic.pdf}}\vspace*{-5pt} 
    \caption{ Average cumulative reward $\bar F_\X$ of the different policies under \WeightedCoverage{} dataset under different setups: stationary in (a) and non-stationary in (b).  Non-stationarity in (b) is applied by changing the objective at $t=25$ (see Appendix~\ref{appendix:experiments}). The area depicts the standard deviation over 5 runs.}\label{fig:dynamicregret}
 %     \vspace*{-2pt}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \subcaptionbox{}{\includegraphics[width = .24\textwidth]{figs/stationary.pdf}}
%     \subcaptionbox{}{\includegraphics[width = .24\textwidth]{figs/dynamic.pdf}}
%     % \subcaptionbox{}{\includegraphics[width = .3\textwidth]{figs/optimistic.pdf}}
%     \caption{ Average cumulative reward $\bar F_\X$ of the different policies under \WeightedCoverage{} dataset under different setups: stationary in (a) and non-stationary in (b)--(c): a reward distribution shift occurs at $t=25$ (see Appendix~\ref{appendix:experiments}).  Non-stationarity in (b) is applied by changing the objective at $t=25$ and in (c) it is applied at every timeslot.  
%     % Subfigure~(c) shows \Algorithm{Optimistic OGA} and \Algorithm{OGA} for different learning rates under different prediction accuracy (noise with std. dev. $n_{\sigma} \in \set{10, 100}$). The larger learning rate is depicted by a solid line. 
%     The area depicts the standard deviation over 5 runs.}\label{fig:dynamicregret}
%       \vspace*{-20pt}
% \end{figure}

==> paper_body.tex <==

\section{Introduction}\label{sec:intro}

 In  online submodular optimization (OSM)~\cite{onlineassignement}, %,harvey2020improved,matsuoka2021tracking}, 
 submodular reward functions 
  chosen by an adversary are  revealed over several rounds. In each round, a decision maker first commits to a set satisfying, e.g., matroid constraints. Subsequently, the reward function is revealed and evaluated over this set. %Due to the setting's combinatorial nature, 
  The objective is to minimize $\alpha$-regret, i.e., the difference of the cumulative reward accrued from the one attained by a static set, selected by an $\alpha$-approximation algorithm operating in hindsight. OSM  has received considerable interest recently, both in the full information \cite{harvey2020improved,matsuoka2021tracking,onlineassignement,niazadeh2021online} and bandit setting \cite{niazadeh2021online,matsuoka2021tracking, wan2023bandit}, where only the reward values (rather than the entire functions) are revealed.


Online convex optimization (OCO) studies a similar online setting in which reward functions are concave, and decisions are selected from a compact convex set. First proposed by Zinkevich~\cite{zinkevich2003}, who showed that projected gradient ascent attains sublinear regret, OCO generalizes previous online problems like  prediction with expert advice~\cite{littlestone94}, and has become widely influential in the learning community~\cite{hazan2016introduction, shalev2012online,mcmahan2017survey}. Its success is evident from the multitude  of OCO variants in literature:  in \emph{dynamic regret} OCO~\cite{zinkevich2003, besbes2015non, jadbabaie2015online, mokhtari2016online}, the regret is evaluated w.r.t.~an optimal comparator sequence instead of an optimal static decision in hindsight. \emph{Optimistic}~OCO~\cite{rakhlin2013online,dekel2017online,mohri2016accelerating} takes advantage of benign sequences, in which reward functions are predictable: the decision maker  attains tighter regret bounds when predictions are correct, falling back to the existing OCO regret guarantees when  predictions are unavailable or inaccurate. \emph{Bandit} OCO algorithms~\cite{hazan2014bandit, kleinberg2004nearly, Flaxman2005} study the aforementioned bandit setting, where again only  rewards (i.e., function evaluations) are observed. 



We make the following contributions:

\begin{packed_itemize}
    \item We provide a methodology for reducing OSM to OCO, when submodular functions selected by the adversary are bounded from above and below by concave relaxations and coupled with an opportune rounding. We prove that algorithms and regret guarantees in the OCO setting  transfer to $\alpha$-regret guarantees in the OSM setting, via a transformation that we  introduce. Ratio $\alpha$ is determined by how well concave relaxations approximate the original submodular functions.
    
    \item We show that the above condition is satisfied by a wide class of submodular functions, namely, \emph{weighted threshold potential} (WTP) functions. This class strictly generalizes weighted coverage functions \cite{karimi2017stochastic,stobbe2010efficient}, and includes many important applications, including influence maximization~\cite{kempe2003maximizing}, facility location~\cite{krause2014submodular,frieze1974cost},   cache networks~\cite{ioannidis2016adaptive,li2021online}, similarity caching~\cite{sisalem2022ascent},  demand forecasting~\cite{ito2016large}, and team formation~\cite{li2018learning}, to name a few.
    
    \item We show our reduction also extents to the dynamic regret and optimistic settings, reducing such full-information OSM settings to the respective OCO variants. To the best of our knowledge, our resulting algorithms are the first to come with guarantees for the dynamic regret and optimistic settings in the context of OSM with general matroid constraints. 
    Finally, we also provide a different reduction for the bandit setting, again for all three (static, dynamic regret, and optimistic) variants; this  reduction applies to general submodular functions, but restricted to partition matroids. 
\end{packed_itemize}
% \replaced[id=GO]{}{
The remainder of the paper is organized as follows. We present related work and a technical preliminary in Sec.~\ref{sec:related} and Sec.~\ref{s:tech_preliminary}, respectively, and define our setting in Sec.~\ref{s:problem}. We state our main results in Sec.~\ref{sec:osmviaoco}, discuss extensions in Sec.~\ref{sec:extensions}. Our experimental results are in Sec.~\ref{sec:experiments}; we conclude in Sec.~\ref{sec:conclusions}.
% }
%removing because sections are not numbered in this format.


% \begin{table*}[!t]
% \resizebox{\textwidth}{!}{
% \begin{tiny}
% \begin{tabular}{||c||c||c|c|c||c|c|c||c|c|c||c|c|c||c||}
% \toprule
%  & \multicolumn{1}{c||}{ \textbf{Prob.}}  &\multicolumn{12}{c||}{\textbf{$(1-1/e)$-regret}} & \\
% \cline{3-14}
% \textbf{Paper}  & \textbf{Class} &\multicolumn{3}{c||}{\textbf{Static/Full Information}}&\multicolumn{3}{c||}{\textbf{Bandit}} &\multicolumn{3}{c||}{\textbf{Dynamic}} & \multicolumn{3}{c||}{\textbf{Optimistic}} &  \textbf{Time} \\
% \cline{3-14}
% &&\textbf{Uni.}&\textbf{Part.}&\textbf{Gen.}&\textbf{Uni.}&\textbf{Part.}&\textbf{Gen.}&\textbf{Uni.}&\textbf{Part.}&\textbf{Gen.}&\textbf{Uni.}&\textbf{Part.}&\textbf{Gen.}&\\
% \cline{1-15}
% \cite{niazadeh2021online} & GS& $r\sqrt{\log\parentheses{n} T}$&\xmark&\xmark& $rn^{\frac{2}{3}} \log^{\frac{1}{3}} (n) T^{\frac{2}{3}} $&\xmark&\xmark&\xmark&\xmark&\xmark&\xmark&\xmark & \xmark & $T^4 O_b$\\
% \hline
% \cite{harvey2020improved}& GS& \multicolumn{3}{c||}{$ \sqrt{r\log\parentheses{\frac{n}{r}} T}$}&\xmark&\xmark&\xmark&\xmark &\xmark &\xmark&\xmark&\xmark&\xmark&\parbox{1.5cm}{ \centering $n r^2 + O_{\mathrm m}\cdot n^4/\epsilon^3$ \\ $\log\parentheses{{n^3 T}/{\epsilon}}$ }\\
% \hline
% \cite{matsuoka2021tracking}  & GS&$r  \sqrt{ r\log(nT) T}$&\xmark&\xmark&\xmark&\xmark &\xmark &$\sqrt{r (r\log(nT) + P_T) T}$&\xmark&\xmark&\xmark & \xmark & \xmark &   ${n r}$\\
% \hline
% \cite{onlineassignement}  & GS & \multicolumn{2}{c|}{$r^{\frac{3}{2}} \sqrt{ \log(n) T} $ }&\xmark&\multicolumn{2}{c|}{$\log^{\frac{1}{3}}(n)(n  c_{\mathrm p} r)^{\frac{2}{3}}T^{\frac{2}{3}}$}& \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  & ${n^2 c_{\mathrm p} }$\\ 
% \hline
% \cite{wan2023bandit}  & GS &\multicolumn{3}{c||}{\xmark}& \multicolumn{2}{c|}{$r^{\frac{4}{3}} n^{\frac{4}{3}}T^{\frac{2}{3}}$}& \xmark & \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $ n r^2$ \\
% \hline
% \hline
% \cite{chen2018online}  & DR-S&\multicolumn{3}{c||}{$\sqrt{rnT}$ }& \xmark & \xmark&\xmark& \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $\sqrt{T} O_{\mathrm {oco}}\cdot O_{\mathrm m}+ n r^2$ \\
% \hline
% \cite{zhang2019online}  & DR-S&\multicolumn{3}{c||}{$T^{\frac{4}{5}}$ }& \multicolumn{3}{c||}{$T^{\frac{8}{9}}$ } & \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $ T^{\frac{3}{5}} O_{\mathrm{oco}}\cdot O_{\mathrm m}+ n r^2 $ \\
% \hline
% \cite{zhang2022stochastic}  & DR-S&\multicolumn{3}{c||}{$\sqrt{rnT}$ }& \xmark & \xmark&\xmark& \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $O_{\mathrm{oco}} \cdot O_{\mathrm m}+ n r^2 $  \\
% \hline
% \hline
% \cite{kakade2007playing}  & LWD&\multicolumn{3}{c||}{$n(\alpha+2) \sqrt{T}$ }& \multicolumn{3}{c||}{$n^{\frac{5}{3}} T^{\frac{2}{3}}$}& \xmark& \xmark&\xmark&\xmark&\xmark&\xmark& $ T O_{\mathrm{\alpha}}$ \\
% \hline
% \hline
% \paintbg \parbox{.25cm}{\centering This\\work}& \parbox{1cm}{\centering\paintbg WTP \\ GS\textsuperscript{$\dagger$}}& \multicolumn{3}{c||}{\paintbg $r\sqrt{\log(\frac{n}{r}) T}$} &  \multicolumn{2}{c|}{\parbox{3cm}{\paintbg \centering $ \alpha r^{5/2} n^{3/2} T^{4/5}$ (dynamic)~\textsuperscript{$\dagger$} \\ $ \alpha r^{4/3} n^{4/3} T^{2/3}$ (static)~\textsuperscript{$\dagger$} }} & \paintbg \xmark & \multicolumn{3}{c|}{\paintbg $\sqrt{r (r\log(\frac{n}{r}) + \log(n) P_T) T}$}&\multicolumn{3}{c|}{\paintbg \parbox{2.7cm}{\centering $\sqrt{r (r\log(\frac{n}{r}) + \log(n) P_T)}t$\\  $\cdot \sqrt{\displaystyle\sum^T_{t =1} \norm{\g_t - \g_t^\pi}_\infty^2}$} }&\paintbg ${n r^2}$\\
% \bottomrule
% \end{tabular}
% \end{tiny}
% }

% \caption{Order ($\BigO{\,\cdot\,}$) comparison of regrets and time complexities attained by different online submodular optimization algorithms for general submodular  (GS) and others for continuous DR-submodular  (DR-S) functions. We also include Kakade et al.~\cite{kakade2007playing}, who operate on Linearly Weighted Decomposable (LWD) functions, and our work on Weighted Threshold Potential (WTP) functions. The footnote (\textsuperscript{$\dagger$}) indicates that  our algorithm extends to GS class in the bandit setting. We also indicate whether algorithms operate over uniform, partition, or general matroid constraints, in the static/full information, bandit, dynamic, and optimistic settings. Regret and complexity are characterized in terms of the time horizon $T$, the  ground set size $n$, the matroid rank $r$. Additional, algorithm-specific parameters are specified in Appendix~\ref{appendix:additional_related_work}.
% % : $C$ the size of color palette, $\vec{\mathcal{A}}_b$ is a Blackwell approachability policy,  $\vec{\mathcal{A}}_{\mathrm{FTRL}}$ is an FTRL policy, $\vec{\mathcal{A}}_{\mathrm{OLO}}$ is an online linear optimization policy, and $\vec{\mathcal{A}}_{\mathrm{OGA}}$ is online gradient ascent. %In the full information setting, all algorithms yield $O(\sqrt{T})$ $\alpha$-regret.
% The SoTA general submodular+general matroid algorithm \cite{harvey2020improved} has a tighter regret than us by a factor $\sqrt{r}$, but has a much higher computational complexity. We attain the same or or better regret than the DR-S \cite{chen2018online,zhang2019online,zhang2022stochastic}  and remaining algorithms, that also either operate on restricted constraint sets \cite{niazadeh2021online,matsuoka2021tracking, onlineassignement} or on the much more restrictive LWD class \cite{kakade2007playing}. In the bandit setting competing algorithms that outperform us either only operate on limited constraint sets \cite{niazadeh2021online,onlineassignement} or the LWD class \cite{kakade2007playing}, while \cite{zhang2019online} attain worse regret; with the exception of the work of~\cite{wan2023bandit} which attains a tighter regret in the static setting over GS class, however when we employ a specialized static OCO algorithm we attain the same bound.  Most importantly, our work readily generalizes to the dynamic and optimistic settings. With the sole exception of \cite{matsuoka2021tracking}, which studies dynamic regret restricted to uniform matroids,  our work is the  first to provide guarantees for online submodular optimization in the dynamic and optimistic settings under general matroid constraints. Leveraging the concave relaxation and eschewing computing the multilinear relaxation also yields significant computational complexity dividends. }
% \vspace*{-15pt}
% \label{table:compare}
% \end{table*}




\section{Related Work}\label{sec:related}
\input{figs/compare}
\noindent\textbf{Offline Submodular Maximization and Relaxations of Submodular Functions.} Continuous relaxations of submodular functions  play a prominent role in submodular maximization. The so-called continuous greedy algorithm~\cite{calinescu2011maximizing} maximizes %a general monotone submodular function subject to a matroid constraint as follows. First, it optimizes 
the multilinear relaxation of a submodular objective over the convex hull of a matroid, using a variant of the Frank-Wolfe algorithm \cite{frank1956algorithm}. The fractional solution is then rounded via pipage \cite{ageev2004pipage} or swap rounding \cite{chekuri2010dependent}, which we also use.  The multilinear relaxation is not convex but is continuous DR-submodular \cite{bach2019submodular,bian2017guaranteed}, and continuous greedy comes with a $1-\frac{1}{e}$ approximation guarantee. However, the multilinear relaxation is generally not tractable and is usually estimated via sampling. 
Ever since the seminal paper by Ageev and Sviridenko~\cite{ageev2004pipage}, several works have exploited the existence of concave relaxations of weighted coverage functions (e.g.,~\cite{karimi2017stochastic,ioannidis2016adaptive}), a strict subset of the threshold potential functions we consider here. For coverage functions, a version of our ``sandwich'' property (Asm.~\ref{assumption:sandwich}) follows directly by the Goemans \& Williamson inequality \cite{goemans1994new}, which we also use.  Both in the standard~\cite{ageev2004pipage} and stochastic offline~\cite{karimi2017stochastic,ioannidis2016adaptive} submodular maximization setting, in which the objective is randomized, exploiting concave relaxations of coverage functions yields significant computational dividends, as it eschews any sampling required for estimating the multilinear relaxation. We depart from both by considering a much broader class than coverage functions and %in 
studying the online/no-regret setting.

%\noindent\textbf{Offline Submodular Maximization.}  A celebrated result by Nemhauser et al.~\cite{nemhauser1978analysis} provides a $(1-1/e)$-approximation  for submodular maximization problems subject to uniform matroid constraints via the greedy algorithm. For general matroids this approximation ratio deteriorates to $1/2$~\cite{fisher1978analysis}. Calinescu et al.~\cite{calinescu2011maximizing} so that the so-called continuous greedy algorithm improves this to a $(1-1/e)$-approximation. Akin to our work, this solves the problem in the continuous domain: continuous greedy finds a maximum of the multilinear extension of the submodular objective using a variant of the Frank-Wolfe algorithm \cite{frank1956algorithm}. The fractional solution is then rounded via pipage \cite{ageev2004pipage} or swap rounding \cite{chekuri2010dependent}. Filmus and Ward \cite{filmus2014monotone} obtain the same approximation ratio through a combinatorial algorithm  requiring no rounding. 
 %
% Several works~\cite{asadpour2008stochastic,karimi2017stochastic,hassani2017gradient,mokhtari2020stochastic, mokhtari2018conditional} consider the \emph{stochastic} submodular optimization setting, in which the objective is random and the aim is to maximize its expectation with access only to independent~function calls: this captures scenarios where exact function evaluation is infeasible for computational or statistical reasons (an example is influence maximization \cite{kempe2003maximizing}).   Hassani et al.~\cite{hassani2017gradient} propose gradient  methods for  general stochastic submodular problems that achieve a $1/2$ approximation guarantee. Mokhtari et al.~\cite{mokhtari2018conditional} improve this to a  $(1-1/e)$-approximation ratio via
%stochastic conditional gradient methods. The online optimization setting we consider here departs both in bounding regret (which requires exploiting while exploring), but also in the non-stochastic evolution of time-variant objectives.

%\noindent\textbf{Concave Relaxations of Submodular Functions.} Ever since the seminal paper by Ageev and Sviridenko~\cite{ageev2004pipage}, several works have exploited the existence of a concave relaxations of weighted coverage functions (see, e.g.,~\cite{karimi2017stochastic,ozcan2021submodular}), a strict subset of the threshold potential functions we consider here. For coverage functions, a version of our ``sandwich'' Lemma~\ref{lemma:util_bounds_lower} follows directly by the Goemans \& Williamson inequality \cite{goemans1994new} (which we also use). Both in the offline~\cite{ozcan2021submodular} and stochastic~\cite{karimi2017stochastic} settings, exploiting concave relaxations of coverage functions yield significant computational dividends. We depart both by considering a much broader class than coverage functions as well as in studying the online/no-regret setting.

%Karimi et al.~\cite{karimi2017stochastic} restrict objectives to a subclass of submodular functions, namely, the weighted coverage functions. They demonstrate that this class admits a concave relaxation method for which  gradient methods can be leveraged to match the $(1-1/e)$-approximation guarantee. They show empirically that this approach reduces the computational cost by orders of magnitude. In this work, we also consider a subclass of submodular objectives (weighted threshold potentials in Sec.~\ref{s:wtp}) which is a strictly more general class than weighted coverage. We deviate from the above works by considering an online setting under time-varying objectives revealed progressively over time.

%\noindent\textbf{Online Submodular Maximization via Regret Minimization.}  As discussed in the introduction, the goal in online submodular optimization problems is to minimize $\alpha$-regret. Typically, $\alpha=1-1/e$ is the approximation guarantee attainable in this setting. \ldots

\noindent\textbf{OSM via Regret Minimization.} Several online algorithms have been proposed for maximizing general submodular functions \cite{niazadeh2021online,harvey2020improved,matsuoka2021tracking,onlineassignement} under different matroid constraints. There has also been recent work~\cite{chen2018online,zhang2019online,zhang2022stochastic} on the online maximization of continuous DR-submodular functions~\cite{bach2019submodular}. Proposed algorithms are applicable to our setting, because the multi-linear relaxation is DR-submodular, and guarantees can be extended to matroid constraint sets again through rounding~\cite{chekuri2010dependent}, akin to the approach we follow here. Also pertinent is the work by~\citet{kakade2007playing}: their proposed online algorithm operates over reward functions that can be decomposed as the weighted sum of finitely many (non-parametric) reference functions--termed Linearly Weighted Decomposable (LWD); the adversary selects only the weights. Applied to OSM, this is a more restricive function class than the ones we study. %Finally, some of these algorithms \cite{niazadeh2021online,onlineassignement,zhang2019online,kakade2007playing} extend to the bandit setting.

We compare these algorithms to our proposed approach in Table~\ref{table:compare}. In the full information setting, the OSM algorithm operating on general matroids by~\citet{harvey2020improved} has a slightly tighter $\alpha$-regret than us, but has a significantly higher computational complexity. We attain the same or better regret than the DR-S \cite{chen2018online,zhang2019online,zhang2022stochastic}  and remaining algorithms, that  either operate on restricted constraint sets \cite{niazadeh2021online,matsuoka2021tracking, onlineassignement} or on the much more restrictive LWD class~\cite{kakade2007playing}.  Most importantly, our work readily generalizes to the dynamic and optimistic settings. With the sole exception of \citet{matsuoka2021tracking}, who studies dynamic regret restricted to uniform matroids,  our work is the  first to provide guarantees for online submodular optimization in the dynamic and optimistic settings under general matroid constraints.

\noindent\textbf{OSM in the Bandit Setting.} Our reduction to OCO in the bandit setting extends the analysis by~\citet{wan2023bandit}, who provide a reduction to just FTRL in the static setting, under general submodular functions and partition matroid constraints. We generalize this to any OCO algorithm and to the dynamic and optimistic settings. Interestingly, \citet{wan2023bandit} conjecture that no sublinear regret  algorithm  exists for general submodular functions under general matroid constraints in the bandit setting. We compare to bounds attained by \citet{wan2023bandit} and other bandit algorithms for OSM \cite{niazadeh2021online,onlineassignement,zhang2019online,kakade2007playing} in Table~\ref{table:compare2} in Appendix~\ref{appendix:bandit:setting}. Our main contribution  is again the extension to the dynamic and optimistic settings. %either only operate on limited constraint sets \cite{niazadeh2021online,onlineassignement} or the LWD class~\cite{kakade2007playing}, while~\citet{zhang2019online} attain worse regret; with the exception of the work of~\citet{wan2023bandit} which attains a tighter regret in the static setting over GS class, however when we employ a specialized static OCO algorithm we attain the same bound. 

%(e.g., pipage \cite{ageev2004pipage} or swap rounding \cite{chekuri2010dependent} in the offline setting or their oblivious randomized versions~\cite{chekuri2010dependent}.
%In online submodular optimization problems, the objective functions are initially unknown and are progressively revealed over $T$ rounds. The goal of the algorithms under this setting is to minimize regret, rather than the optimization error. When the objective functions are stochastic and i.i.d. such a setting is called \emph{stochastic} online submodular maximization~\cite{chen2018projection}, and when the objective functions are  are arbitrary or even adversarial, this setting is called online \emph{adversarial} submodular maximization, or simply online submodular maximization~\cite{streeter2008online,onlineassignement}.  Streeter et al.~\cite{streeter2008online} present an online greedy algorithm, combining the greedy algorithm with no-regret algorithm operating over a  probability simplex and under uniform matroids, and then extended their results to partition matroids~\cite{onlineassignement}. Radlinski et al. \cite{radlinski2008learning} propose  an online algorithm for unifrom matroid by running a separate instance of a multiarmed bandit algorithm for each step of the greedy algorithm. Chen et al. \cite{chen2018projection} use Stochastic Continuous Greedy \cite{mokhtari2018conditional} to achieve sublinear $(1-1/e)$-regret bound without projections and exact gradient. Niazadeh et al.~\cite{niazadeh2021online} propose a framework to transform offline robust greedy algorithms to online ones using Blackwell approachability to obtain sublinear $(1-1/e)$-regret. Harvey et al.~\cite{harvey2020improved} propose an algorithm whose fractional decisions are obtained by exerting a continuous-time dynamics over the output of multiple instances of online dual averaging policies; the fractional decisions of the algorithm are rounded to obtain sublinear $(1- 1/e)$-regret.  Our approach departs significantly from these interesting works in that we employ a concave relaxation  that provides clear separation of the continuous and integral domains; moreover,  the link between the two domains is established through randomized rounding. We demonstrate that the framework of OCO and its flavours can be leveraged to design policies that are computationally efficient with optimized regret constants; this allows us to bring the rich flavours of OCO (e.g., dynamic regret, bandit, optimistic learning) to the online submodular maximization problem. Table~\ref{table:compare}  summarizes the regret guarantees attained by our approach and its time complexity compared to related work.

%\noindent\textbf{Online DR-Submodular Maximization via Regret Minimization.} 
%Recently, continuous DR-submodular functions have been proposed as a broad class of non-convex functions, which exhibit diminishing returns property. This class is an extension of the definition of submodularity to continuous domains~\cite{bach2019submodular}.  Bian et al.~\cite{bian2017guaranteed} building on the continuous greedy of Calinescu et al.~\cite{calinescu2011maximizing} proposes a policy that provides a $(1-1/e)$-approximation algorithm for maximizing monotone continuous DR-submodular functions subject to down-closed convex constraints. Hassani et al.~\cite{Hassani2020} and Mokhtari~\cite{mokhtari2018conditional} proposed improved variants of the continuous greedy algorithm combined  with variance
%reduction techniques of stochastic gradients. Several works~\cite{chen2018online,zhang2019online} study online DR-submodular maximization. Chen et al. \cite{chen2018online} convert the offline Frank-Wolfe variant/continuous greedy  to a no-regret online algorithm, obtaining a sublinear $(1-1/e)$-regret. Zhang et al.~\cite{zhang2022stochastic} propose a a boosting framework for online gradient ascent,  obtaining a sublinear $(1-1/e)$-regret. This line of work can be applicable to our setting, because the multi-linear relaxation of a submodular objective is DR-submodular; algorithms that provide guarantees under this continuous setup can be extended to have guarantees over matroid constraint sets though rounding (e.g., pipage \cite{ageev2004pipage} or swap rounding \cite{chekuri2010dependent} in the offline setting or their oblivious randomized versions~\cite{chekuri2010dependent} in the online setting). However, the multi-linear extension can be computationally expensive (as it may involve $2^n$ terms), and constructing noisy estimates of its gradients introduces variance to the learning process. In this work, we consider a different approach based on a concave relaxation approach that does not require the multilinear extension. 

%\noindent\textbf{Online Convex Optimization.}
%Online convex optimization (OCO)  was first proposed by Zinkevich~\cite{zinkevich2003online}, who showed that projected gradient descent attains sublinear regret bounds in the online setting. OCO generalizes previous online problems like the prediction with expert advice problem~\cite{littlestone94}, and has become widely influential in the learning community~\cite{hazan2016introduction, shalev2012online,mcmahan2017survey}. Different flavours  of OCO were also considered in the literature.  In dynamic regret~\cite{zinkevich2003online,besbes2015non,jadbabaie2015online,mokhtari2016online}, the regret the policy is evaluated w.r.t. a comparator sequence instead of a single decision as in the static regret. In bandit convex optimization (BCO)~\cite{hazan2014bandit,kleinberg2004nearly,flaxman2004online}, the decision maker observes the concave reward function only at the decision that he has chosen. Optimistic OCO~\cite{rakhlin2013online} was introduced to take advantage of benign sequences, under which the decision maker can enjoy tighter regret bounds as compared to the typical worst case bounds when the rewards are predictable; moreover, when the predictions are unavailable or inaccurate the worst-case guarantees are preserved.



\section{Technical Preliminary}
\label{s:tech_preliminary}

\noindent\textbf{Submodularity and Matroids.}
   Given a ground set $V=[n]\triangleq \set{1,2,\dots, n}$, 
a set function $f: 2^V \to \reals$ is \emph{submodular} if  $f(S \cup \set{i, j}) - f(S \cup \set{j})  \leq  f(S \cup \set{i}) - f(S)$ for all $S \subseteq V$ and $i,j \in V \setminus S$ and \emph{monotone} if    $f(A) \leq f(B)$  for all $A \subseteq B \subseteq 2^V$. %Given a vector $\x \in \reals^n$, we denote its support by  $\supp{\x} \triangleq \set{i \in V: x_i\neq 0}$.
%
A \emph{matroid} is a pair $\M = (V, \I)$, where  $\I \subseteq  2 ^{V}$, %is the set of \emph{independent} sets,
for which the following holds:  (1) if $B \in \I$ and $A \subseteq B$, then $A \in \I$, %which implies $\emptyset \in \I$, (downward-closed property), 
(2) if $A, B \in \I$ and $\card{A} < \card{B}$, then there exits an $x \in B \setminus A$ s.t. $A \cup \set{x} \in \I$. %(independent set exchange property). 
The \emph{rank} $r \in \naturals$ of $\M$ is the cardinality of the largest set in $\I$. 
 With slight abuse of notation, we  represent set functions $f: 2^V \to \reals$  as functions over $\{0,1\}^n$: given a set function $f$ and an $\x\in\{0,1\}^n$, we denote by $f(\x)$ as the value $f(\supp{\x})$,  where  $\supp{\x} \triangleq \set{i \in V: x_i\neq 0} \subseteq V$ is the support of $\x$. Similarly, we treat matroids as subsets of  $\{0,1\}^n$.  %We denote  by $\conv{S}$ the convex hull of a set $S \subset  \reals^n$; for a matroid $\M\subseteq \{0,1\}^n$. %, $\conv{\M}$ is known as the \emph{matroid polytope} of $\M$.

%We first  describe the general protocol of {full-information} online learning.


% \paragraph{Threshold Potentials.} Given a ground set $V$, a set $S \subseteq V$, weight vector $\vec w = (w_i)_{i \in S}$ for  $w_i \in \reals_{\geq 0}$, and a threshold $b \in \reals_{\geq 0}$, the threshold potential  set function $\Psi_{b,\vec w, S}: \set{0,1}^n \to \reals_{\geq 0}$ is defined as 
% \begin{align}
%     \Psi_{b,\vec w, S} (\x) &\triangleq  \min\set{b, \sum_{i \in S} w_i x_i}. & &\text{for $\x \in \set{0,1}^n$.}\label{eq:threshold_potential}
% \end{align}


 \noindent\textbf{Online Learning.} \label{s:online_learning}
 In the general protocol of \emph{online learning} \cite{cesabianchi2006}, a decision-maker makes sequential decisions and incurs rewards as follows: %sequentially; after every decision a reward is accrued, and decisions can only depend on past observations. Formally, 
 at timeslot $t \in [T]$, where $T\in \naturals$ is the time horizon, the {decision-maker} first commits to a decision $\x_t \in \X$ from some set $\X$. Then, a reward function  $f_t:\X\to\reals_{\geq 0}$ is selected by an adversary from a set of functions $\F$ and revealed  to the decision-maker, who accrues a reward $f_t(\x_t)$.  The decision $\x_t$ is determined  according to a (potentially random) mapping  $\P_{\X,t}: \X^{t-1} \times  \F^{t-1}\to \Y$, i.e., 
 \begin{align}\label{eq:onlineprotocol}
     \x_{t} = \P_{\X, t} \parentheses{\parentheses{\x_s}^{t-1}_{s=1} , \parentheses{f_s}^{t-1}_{s=1}} .
 \end{align}
Let $\vec\P_\X = (\P_{\X,t})_{t \in \T}$ be the \emph{online policy} of the decision-maker. 
 % The decision maker starts initially with a feasible decision $\x_1 \in \X$.
We define the \emph{regret} of  $\vec\P_\X$ at horizon $T$ as:
\begin{equation}
    \begin{split}
        \mathrm{regret}_T ({\vec\P}_\X)  
     \triangleq  \sup_{({f}_t)_{t=1}^{T}  \in {\F}^T}  \bigg\{ \max_{\x\in \X}  \sum^T_{t=1} {f}_t(\x) -\underset{{{\vec\P}_\X}}{\E}\left[\sum^T_{t=1}{f}_t(\x_t)\right]\bigg\} \label{eq:general_regret}.
    \end{split}
\end{equation}
%where the expectation is over the randomization of  $\vec\P_\X$. In general, 
We seek policies that attain a sublinear (i.e., $o(T)$) regret; intuitively, such policies  perform on average as
well as the static optimum in hindsight.
%
Note that the regret is defined w.r.t.~the optimal \emph{fixed} decision $\x$, i.e., the time-invariant decision $\x\in \X$ that would be optimal in hindsight, after the sequence $(f_t)_{t=1}^{T}$ is revealed. When selecting  $\x_t$, the decision-maker has no information about the upcoming reward $f_t$. Finally, this is the \emph{full-information} setting: at each timeslot, the decision maker observes the entire reward function $f_t(\,\cdot\,)$, rather than just the reward $f_t(\x_t)\in \reals_{\geq 0}$.

Deviating from these assumptions is of both practical and theoretical interest. %, and has indeed been  considered in the literature. In particular, 
In the \emph{dynamic regret} setting \cite{zinkevich2003}, the regret is measured w.r.t. a time-variant  optimum, appropriately constrained so that changes from one timeslot to the next do not vary significantly. 
In  \emph{learning with optimism}  \cite{rakhlin2013online}, additional information is assumed to be available w.r.t. $f_t$, in the form of so-called predictions. In the \emph{bandit} setting \cite{auer1995gambling}, the online policy ${\vec\P}_\X$ of the decision maker only has access to rewards $f_t(\x_t)\in \reals_{\geq 0}$, as opposed to the entire reward function.  %We provide  formal definitions of all three settings in Sections~\ref{s:dynamic}, \ref{s:bandit}, and~\ref{s:optimism}, respectively, as our work also extends to these settings.

\paragraph{Online Convex Optimization.} The \emph{online convex optimization} (OCO) framework~\cite{zinkevich2003, hazan2016introduction} follows the above online learning protocol~\eqref{eq:onlineprotocol},  where (a) the decision space $\X$ is a  convex set in $\reals^n$, and (b) the set of reward functions $\F$ is a subset of concave functions over $\X$.  %selected by an adversary from some set $\hat \F$. At timeslot $t \in \T$, a decision $\y_t$ is determined according to a mapping $\P_{\Y,t}: \Y^{t-1} \times  \hat{\F}^{t-1}\to \Y$, i.e.,
%\begin{align}
  %  \y_{t} =\P_{\Y,t} \parentheses{{(\y_s)}^{t-1}_{s=1} , {(\cfunc_s)}^{t-1}_{s=1}}. 
%\end{align} 
Formally, OCO operates under the following  assumption:
\begin{assumption}
    The decision set  $\X \subset \reals^n$ is   closed, bounded, and convex. %with bounded diameter. %We denote by $D$ the upper bound on the diameter of $\Y$:  $\forall \y,\y' \in \Y, \norm{\y - \y'}\leq D$.\label{assumption:convex}
%\end{assumption}
%\begin{assumption}\label{asm:oco}
     The reward functions in $\F$ are all $L$-Lipschitz concave functions w.r.t. a norm $\norm{\,\cdot\,}$ over $\X$, for some common $L\in \reals_{>0}$. % or equivalently~\cite[Lemma 2.6]{shalev2012online}, the dual norms  $\norm{\,\cdot\,}_\star$ of the supergradients of the reward function in $\hat\F$ are bounded by $L$ over $\Y$. 
     \label{asm:oco}
\end{assumption}
There is a  rich literature on OCO policies \cite{hazan2016introduction}; examples  include Online Gradient Ascent (OGA)~\cite{hazan2016introduction}, Online Mirror Ascent (OMA)~\cite{bubeck2011introduction}, and Follow-The-Regularized-Leader (FTRL)~\cite{mcmahan2017survey}. All three enjoy sublinear regret: %; in particular, the following theorem holds:
\begin{theorem} Under Asm.~\ref{asm:oco} OGA, OMA,  and FTRL attain $O(\sqrt{T})$ regret. \label{thm:oco}
\end{theorem}
We provide a detailed description of all three algorithms, as well as formal statements of the regret they attain, in \fullversion{Appendix~\ref{appendix:oco} of the supplement}{Appendix~\ref{appendix:oco}}. %Though all three policies attain $O(\sqrt{T})$ regret, both the constants appearing in this term as well as the  computational and space complexity differ across policies. In general, the optimal policy may be problem dependent; parameters that matter include the diameter of $\X$, the Lipschitz parameter $L$, as well as the norm $\|\cdot\|$ in Asm.~\ref{asm:oco}. %We give a more thorough overview of such issues in \fullversion{Supplementary Material}{Sec.~\ref{s:setups_omd}}.  
%
Most importantly, the OCO framework readily generalizes to %interesting and important variants of the full information setting, determined by Eqs.~\eqref{eq:onlineprotocol}--\eqref{eq:general_regret}. These include 
the   dynamic,  learning-with-optimism, as well as  bandit  settings (see also Sec.~\ref{sec:extensions}). %: OCO policies readily generalize to all of these settings, and come with appropriate regret guarantees (see Sec.~\ref{s:dynamic}--\ref{s:optimism}). 

\noindent\textbf{Weighted Threshold Potentials.} A \emph{threshold potential}~\cite{stobbe2010efficient} $\Psi_{b, \vec{w}, S}: \set{0,1}^n \to \reals_{\geq 0}$, also known as a \emph{budget-additive function} \cite{andelman2004auctions, dobzinski2016breaking,buchfuhrer2010inapproximability}, is defined as: %, have numerous applications in the context of combinatorial auctions~\cite{andelman2004auctions, dobzinski2016breaking,buchfuhrer2010inapproximability}, online advertising~\cite{AdWords,mehta2013online}, and market equilibrium~\cite{roughgarden2015prices,bei2019earning,garg2018approximating,feldman2013combinatorial}.
%\label{s:wtp}
%We define  a threshold potential  $ as
\begin{align}
      \Psi_{b,\vec w, S}(\x)&\triangleq   \min\set{b, \sum_{j \in S} x_j w_j},\,\text{for $\x \in \set{0,1}^n$}, \label{eq:budget-additive}
\end{align}
where   $b \in \reals_{\geq 0} \cup \set{\infty}$ is a threshold,  $S \subseteq V$ is a subset of $V=[n]$, and  $\vec w = (w_j)_{j \in S}\in [0,b]^{|S|}$ is a weight vector bounded by $b$.\footnote{Assumption $ w_{j} \leq b$, $j \in S$, is w.l.o.g., as  replacing $w_{j}$ with $\min\set{w_{j}, b}$ preserves  values of $f$ over  $\set{0,1}^n$.}  The linear combination of threshold potential functions defines the rich class of \emph{weighted threshold potentials} (WTP)~\cite{stobbe2010efficient}, %$f: \set{0,1}^n \to \reals_{\geq 0}$, 
defined as: 
\begin{align}
   f(\x)  & \triangleq \sum_{\ell \in C} c_{\ell} \Psi_{b_\ell,\vec w_\ell, S_\ell} (\x), \quad \text{for $\x \in \set{0,1}^n$},
   \label{eq:wtp}
\end{align}
where $C$ is an arbitrary index set and $c_{\ell} \in \reals_{\geq 0}$, for $\ell\in C$.  WTP functions are submodular and monotone (see Appendix~\ref{appendix:WTP}). %\cite{stobbe2010efficient,dobzinski2016breaking} and \fullversion{Appendix~\ref{appendix:WTP}}{Appendix~\ref{appendix:WTP}}).
We define the \emph{degree} of a WTP function $\Delta_f = \max_{\ell \in C} |S_\ell|$ as the maximum number of variables that a threshold potential $\Psi$ in $f$ depends on.
%$b_{\ell} \in \reals_{\geq 0} \cup\set{\infty}$, $w_{i,j} \in (0,b_i]$, $S_{\ell}\subseteq V$,  $j \in S_i$, and $\ell \in C$, are parameters of the function.
%Examples of a WTP functions are weighted coverage  (WC) functions~\cite{xxx}, given by:
%\begin{align}\label{eq:WCF0}
% $  f(\x) =\sum_{\ell \in C} c_i \min \left\{1, \sum_{\ell \in S_\ell} x_j\right\},$
%\end{align}
%but include many more interesting 
%applications, including influence maximization \cite{xxxx}, quadratic set functions \cite{xxx}, cache networks \cite{xxx}, and similarity caching  \cite{xxx}, to name a few; we review all these in detail in Sec.~\ref{s:applications}. We note that the class 


We give several examples of WTP functions in \fullversion{Appendix~\ref{appendix:WTP}}{Appendix~\ref{appendix:WTP}}. In short, classic problems such as 
 influence maximization~\cite{kempe2003maximizing} and facility location~\cite{krause2014submodular,frieze1974cost},  resource allocation problems like cache networks~\cite{ioannidis2016adaptive,li2021online} and similarity caching~\cite{sisalem2022ascent}, as well as demand forecasting~\cite{ito2016large} and team formation~\cite{li2018learning}  can all be expressed using WTP functions. %They also map very well to the online submodular maximization setting we study here. 
 Overall, the WTP class is very broad: there exists a hierarchy among submodular functions, including weighted coverage functions~\cite{karimi2017stochastic}, weighted cardinality truncations~\cite{dolhansky2016deep}, and sums of concave functions composed with non-negative 
modular functions~\cite{stobbe2010efficient}; all of them are strictly dominated by the WTP class (see~\citet{stobbe2010efficient}, as well as \fullversion{Appendix~\ref{appendix:WTP}}{Appendix~\ref{appendix:WTP}}).  





%\section{Applications} %(Delegated to G. Özcan and I. Nikolaou)
%\label{s:applications}
%In this section, we look at specific examples of WTP functions that can be handled by our framework. 

\iffalse
\noindent\emph{Example 1: Weighted Coverage Functions.}
Classic problems such as 
 influence maximization~\cite{kempe2003maximizing} facility location~\cite{krause2014submodular,frieze1974cost} can all be expressed via the maximization of weighted coverage functions subject to matroid constraints (see~\cite{Karimi2017}). Another such example is cache networks~\cite{ioannidis2016adaptive}, which have also been studied in the online setting~\cite{li2021online}.  
 For $V =[n]$, let $\{S_\ell
\}_{\ell \in C}$ be a collection of subsets of $V$, and $c_\ell \in \reals_{\geq 0}$ be a weight associated to each subset $S_\ell$. A weighted set coverage function $f: \{0, 1\}^n \rightarrow \reals_{\geq 0}$ receives as input an $\x$ representing a subset of $V$ an accrues reward $c_\ell$ if $S_\ell$ is ``covered'' by an element in $\x$: formally,  $f(\x) = \sum_{\ell \in C} c_\ell \left(1 - \prod_{j \in 
    S_\ell} (1-x_j)\right)$. %,  where $\x$ is subject to a matroid constraint. 
\begin{observation}  
    The weighted coverage function $f$ 
   belongs to the class of WTP functions described by~\eqref{eq:wtp}; in particular:
  $f(\x) = \sum_{\ell \in C} c_{\ell} \Psi_{1, \vec 1, S_\ell} (\x)$ for every $\x \in \set{0,1}^n$.
\end{observation}
Our online setting naturally captures different epidemics over the same graph in influence maximization and dynamic tasks in facility location~\cite{Karimi2017}, as well time-variant file requests in cache networks~\cite{li2021online}.
\fi
\iffalse    
Weighted coverage models various applications such as influence maximization~\cite{kempe2003maximizing}, facility location~\cite{karimi2017stochastic}, and cache networks~\cite{ioannidis2017jointly}.  In influence maximization, the goal is to maximize the expected fraction of nodes reached if we start by infecting seeds $S \subseteq V$ and the infection spreads with the Independent Cascade model (IC) model \cite{kempe2003maximizing}. Given a directed graph $G = (V, E)$, where $V = [n]$ is a set of nodes of instance $G$, the fraction of nodes that are reachable from $S$ using the edges $E$ can be formulated as $f_G(\x) = \frac{1}{n}\sum_{v \in V}\left(1 - \prod_{i \in P_v}(1-x_i)\right)$, where $P_v \subseteq V$ is the set of nodes reachable from $v$ in a in a stochastic instance of the IC model. Therefore, $f_G(\x)$ is a weighted coverage function and hence a weighted threshold function in the form $f_G(\x) = \frac{1}{n} \sum_{v \in V} \Psi_{1, \vec 1, P_v} (\x)$. Facility location problems can be also expressed as weighted coverage functions \cite{karimi2017stochastic} and hence, weighted threshold potential functions. Given a complete weighted bipartite graph $G = (V, M)$ and weights $w_{i, j} \in [0, 1]$, $i \in V$, $j \in M$, the objective is to maximize $f_j (S) = \max_{i \in S} w_{i, j}$, where $V$ and $M$ represent facilities and customers respectively and $w_{i, j}$ represent the utility of facility $i$ for customer $j$. Karimi et al. \cite{karimi2017stochastic} makes the following observation $ f_j(\x) = \sum_{\ell=1}^N (w_{i_{\ell}, j} - w_{i_{\ell+1}, j}) \left(1 - \prod_{k = 1}^\ell (1 - x_{i_k})\right)$,  where for all $j \in M$, the weights have been sorted in a decreasing fashion as $w_{i_1, j} \geq \ldots \geq w_{i_n, j}$ and $w_{i_{n+1}, j} \triangleq 0$. It is easy to observe that $f_j(\x)$ is a weighted threshold function in the form $f_j(\x) = \sum_{\ell=1}^N (w_{i_{\ell}, j} - w_{i_{\ell+1}, j}) \Psi_{1, \vec 1, S_{\ell}} (\x)$, where $S_{\ell} = \{1, \ldots, \ell\}$.
\fi

\iffalse
\noindent\emph{Example 2: Similarity Caching.} Similarity caching~\cite{sisalem2022ascent} is an extension of the so-called paging problem~\cite{XXXX}.
The objective is to efficiently use local storage memory and provide approximate (similar) answers to a query in order to reduce retrieval costs from some distant server. Formally,
consider a catalog of files  represented by the set $V = [n]$, and an augmented catalog represented by the set $\hat{V} = [2n]$.  Item $i \in V$ is the local copy of a remote file $i+n \in \hat V$. Let $c(i,i') \in \reals$ be the cost of responding to query $i \in V$ with a similar file $i' \in \hat V$. \citet{sisalem2022ascent} show that the reward received under under this setting is given by $ f(\x) = \sum_{l=1}^{C_r - 1} \parentheses{c(r, \pi_{l+1}^r) - c(r, \pi_l^r)} \min \left\{k - \card{S_l}, \sum_{j \in [l] \setminus S_l} x_{\pi_j^r} \right\},$ for some $C_r \in \naturals$, subset $S_l \subset V$ where $\card {S_l}< k$, and permutation $\vec\pi^r: \hat V \to \hat V$ satisfying $c(r, \pi_{l+1}^r) - c(r, \pi_l^r) \geq 0 $ for $l \in [C_l]$. This is indeed a WTP function:
\begin{observation}
The similarity caching objective belongs to the class of WTP functions defined by Eq.~\eqref{eq:wtp}. In particular, $f(\x) = \sum^{C_r}_{l=1}  \parentheses{c(r, \pi_{l+1}^r) - c(r, \pi_l^r)}  \Psi_{ k - \card{S_l},\vec 1, S_l} (\x)$. 
\end{observation}
Note that the above functions cannot be captured by weighted coverage.
\fi
\iffalse
\noindent\emph{Quadratic Set Functions.}  
Motivated by applications such as 
price optimization on the basis of demand forecasting~\cite{ito2016large}, detection
in multiple-input multiple-output channels in communication systems~\cite{MIMO} and team formation~\cite{}, we consider quadratic 
functions $f: \{0, 1\}^n \rightarrow \reals_{\geq 0}$ of the form $f(\x) = \vec{h}^\intercal \x + \frac{1}{2}\x^\intercal \vec{H}\x$.
We focus on functions where $\H$ is symmetric  (with zeros in the diagonal) and entries $\H_{ij}$. Note that $f$ is monotone and submodular if and only if : (a) $\H \leq \vec{0}_{n \times n}$, and (b) $\h + \H \x \geq \vec{0}_{n \times 1}$.
\begin{observation}
The quadratic function $f$  belongs to the class of WTP functions~\eqref{eq:wtp}, i.e.,
 $f(\x) =  \Psi_{\infty,  \h + \H \vec{1}, [n]}(x) +
    \sum_{i=1}^{n-1} \sum_{j=i+1}^n
        (-\H_{ij}) \Psi_{1, \vec{1}, \set{i,j}}(\x)
$, for every $\x\in\set{0,1}^n$.
\end{observation}
\fi

\iffalse
when (a) the matrix $\H$ has non positive entries, i.e. $\H \leq \vec{0}_{n \times n}$, and (b) the gradient of $f$ at any point $\x \in \mathrm{conv}(\X)$ is non-negative, i.e. $\h + \x^\intercal \H \geq \vec{0}_{n \times 1}$. It holds that $f(\x) = (\h + \H\vec{1})^\intercal \x +
                \sum_{i=1}^{n-1} \sum_{j=i+1}^n
                (-H_{i,j}) \min \{1, x_i + x_j\}$ for $\x \in \set{0,1}^n$ (see the proof in Sec. \ref{appendix: quadratic}). Note that alternative formulation permits us to express $f$ in terms of threshold potentials. In particular, it holds that  $ f(x) = \cfunc(\x) \triangleq \Psi_{\infty,  \h + \H \vec{1}, [n]}(x) +
    \sum_{i=1}^{n-1} \sum_{j=i+1}^n
        (-H_{i,j}) \Psi_{1, \vec{1}, S_{i,j}}(x)$, where $S_{i,j} = \{i, j\}$.
\fi

% \emph{Team formation.}
% Let $V = [n]$ be a set of individuals, and consider the problem of constructing a team of individuals $\x = \vec{1}_S$, where $S \subseteq V$ is the selected subset of individuals, such that $\x$ satisfies some matroid constraints. The goal is to maximize the following monotone and submodular function
% \begin{equation}
%     f(\x) = \vec{h}^\intercal \x + \frac{1}{2}\x^\intercal \vec{H}\x, 
% \end{equation}

\iffalse
This type of quadratic set functions model various applications such as team formations~\cite{anagnostopoulos2012online, lappas2009finding, vombatkere2023balancing}, large-scale price optimization on the basis of demand forecasting models~\cite{ito2016large}, detection
in multiple-input multiple-output channels in communication systems~\cite{MIMO}. For instance, in  team formation, the linear term   $\h^\intercal \x$ captures the performance of each individual while the quadratic term $\x^\intercal \H \x$ captures
pairwise effects. 
\fi

% Team formation has been studied in many different settings with various objective functions and constraints \cite{anagnostopoulos2012online, lappas2009finding, vombatkere2023balancing}. 

% None of these works have considered a quadratic objective function to measure team performance.

% \paragraph{Cache Networks.} 
% Consider a network represented as a directed, symmetric graph $G(V, E)$. 
% In the source routing setup described by \cite{ioannidis2017jointly}, the cost of serving a request is  $
    % C_{SR}^{(i, s)}(r, X) = \sum_{p \in \mathcal{P}_{i, s}} r_{(i, s), p}\sum_{k=1}^{|p|-1} w_{p_{k+1}p_k} \prod_{k'=1}^{k}(1-x_{p_k'i}),$
% Given service rates $\mu_j$, $j \in E$, storage capacities $c_v$, $v \in V$, a set of requests $\mathcal{R}$, and arrival rates $\lambda_r$, for $r \in \mathcal{R}$, 

% Consider a network represented as a directed, symmetric graph $G(V, E)$. files can be stored at 
% Ioannidis and Yeh  \cite{} that the reward of file placement under cache networks 


% % The traffic load on an edge $e = (u, v)$ is given by
% \begin{equation} \label{eq:CNgi}
%     \rho_{(u, v)}(\vec{x}) = \frac{1}{\mu_{u, v}}\sum_{r \in \mathcal{R}:(v, u)\in p^r} \lambda^r \prod_{k'=1}^{k_{p^r}(v)}(1-x_{p_k^r, i^r}),
% \end{equation}
% where $\vec{x}\in \{0,1\}^{|V||\mathcal{C}|}$ is a vector of binary coordinates $x_{vi}$ indicating if $i\in \mathcal{C}$ is stored in node $v\in V$. If $\rho_e$ is the load on an edge,  the expected total number of packets in queue $e \in E$ is given by $C_e(\rho_e)=\frac{\rho_e}{1-\rho_e}$. In cache optimization, the objective is to determine placements that solve problems in the following form:
% \begin{equation}
%     \min_{\vec{x} \in \mathcal{D}_{\vec{\lambda}}  }
%     C(\vec{x}) = \sum_{e \in E} C_e (\rho_e(\vec{x})),
% \end{equation}
% where $C_e: [0, 1) \to \mathbb{R}_+$ are positive cost functions, $\rho_e: \mathcal{D} \times \mathbb{R}_+^{|\mathcal{R}|} \rightarrow \mathbb{R}_+$ is the load on edge $e$ and $\mathcal{D}_\vec{\lambda}$ is the set of feasible placements that ensure stability.

% Let us define $f_{(u, v)}(\vec{x}) \triangleq \left(\sum_{r \in \mathcal{R}:(v, u)\in p^r} \frac{\lambda^r}{\mu_{u, v}}\right) - \rho_{(u, v)} (\x)$. Then we can express $f_{(u, v)}(\vec{x})$ as
% \begin{equation}
%     f_{(u, v)}(\vec{x}) = \sum_{r \in \mathcal{R}:(v, u)\in p^r} \frac{\lambda^r}{\mu_{u, v}} \left(1 - \prod_{k'=1}^{k_{p^r}(v)}(1-x_{p_k^r, i^r})\right).
% \end{equation}
% As a result, we can express $f_{(u, v)}(\vec{x})$ as both a weighted coverage function and a weighted threshold potential.



% \textcolor{blue}{Coverage functions + G\"ozde taylor's expansion shouldn't exit the class of coverage functions. It would be nice to check this statement and provide a proof to it. It necessary to do this step to be able to say something about IM problem, since it includes a $\log(1 + \,\cdot\,)$}

% \paragraph{Data Summarization.} 



% Adding the constant $\sum_{i=1}^{K^r-1} \alpha_i^r\sigma_i^r$, on both sides of Eq.~(\ref{eq:simCachGain}) and define $G(r, \x, \vec{\sigma}) \triangleq G(r, \x) + \sum_{i=1}^{K^r-1}$, we obtain
% \begin{equation} \label{eq:simCachGainEdited}
%     G(r, \x, \vec{\sigma}) = \sum_{i=1}^{K^r - 1} \alpha_i^r \min \left\{k, \sum_{j =1}^i x_{\pi_j^r}\right\}.
% \end{equation}
% From Eq.(\ref{eq:simCachGainEdited}), it is easier to see that similarity caching gain function is also a threshold potential function in the form:
% \begin{equation}
%     G(r, \x, \vec{\sigma}) = \sum_{i=1}^{K^r - 1} \alpha_i^r \Psi_{k,\vec 1, S_i} (\x),
% \end{equation}
% where $S_i = \{\pi_1^r, \ldots, \pi_i^r\}$.




%\begin{proposition}
%The set function $f$ in Eq.~\eqref{eq:budget-additive} is submodular and monotone.\label{proposition:subadditive_submodularity}
%\end{proposition}

% The rich class of WTP functions are more expressive and it strictly generalizes weighted coverage functions (WC)~\cite{karimi2017stochastic}, weighted cardinality truncations (WCT)~\cite{dolhansky2016deep}, and sums of concave functions composed with non-negative 
%modular functions 
% (SCM)~\cite{stobbe2010efficient}. We provide in detail the inclusion relationships Sec.~\ref{s:generality_wtp}. %We provide a thorough description of applications captured in this class such as influence maximization, quadratic set functions, cache networks, and similarity caching in Sec.~\ref{s:applications}. 

% Bilmes~\cite{dolhansky2016deep}, and the strict inclusion $\mathrm{SCMM} \subset \mathrm{WTP}$ was shown by Stobbe and Krause~\cite{stobbe2010efficient}.
%\paragraph{The regret  Performance Metric.} The performance metric of interest under the OCO setting is  regret, i.e., the difference between the accrued rewards of the fixed decision in hindsight and that of the decisions taken by the policy. The  OCO framework gives rise to efficient online algorithms with sublinear regret over $T$ iterations, which implies that on average the policy attains asymptotically rewards that compete with the best fixed decision in hindsight. Examples of such policies with provable sublinear regret include: online gradient descent (OGD)~\cite{hazan2016introduction}, online mirror descent (OMD)~\cite{bubeck2011introduction}, follow the regularized leader (FTRL)~\cite{mcmahan2017survey}. All these algorithms enjoy $\BigO{\sqrt{T}}$ regret. Formally, the regret of an OCO policy $\vec{\P}_{\Y}$ after $T$ timeslots is defined as follows:
%\begin{align}
%    \mathrm{regret}_T ({\vec\P}_\Y) \triangleq  %\sup_{\parentheses{\cfunc_1 ,\cfunc_2, \dots, \cfunc_T} \in %\hat{\F}^T}  \set{ \max_{\y\in \Y}  \sum_{t\in\T} \cfunc_t(\y) -\sum_{t \in \T} \cfunc_t(\y_t)} \label{eq:oco_regret}.
%\end{align}




% ?\begin{definition} (Vectorized Set Functions) Given a ground set $V$, the vectorized set function $f: \set{0,1}^V \to \reals$ associated to $f: 2^V \to \reals$ is defined for every $\x \in \set{0,1}^V$ as  $ f(\x) \triangleq f(\supp{x})$.
% With slight abuse of notation 
% \end{definition}



% \section{Problem Formulation} 
% \subsection{}

\section{Problem Formulation}
\label{s:problem}
We consider a combinatorial version of the online learning protocol defined in Eq.~\eqref{eq:onlineprotocol}.  In particular, we focus on the case where (a) the decision set is $\X \subseteq \set{0,1}^n$, i.e., the vectorized representation of subsets of $V=[n]$, and (b) the set $\F$ of reward functions comprises set functions over $\X$. Though some of our results (e.g., Thm.~\ref{theorem:sandwich}) pertain to this general combinatorial setting, we are particularly interested in the case where (a)  $\X$ is a matroid, and (b) $\F$ is the WTP class, i.e., the set of functions whose form is given by Eq.~\eqref{eq:wtp}.


Both in the general combinatorial setting and for WTP functions,  evaluating  the best fixed decision  may be computationally intractable even in hindsight, i.e., when all reward functions were revealed.  %For example, when $\F$ is the set of submodular monotone set functions~(see Sec.~\ref{s:submodularity_matroids}), it is  NP-hard to evaluate any $(1 - 1/e + \epsilon)$-approximation of the offline optimum for $\epsilon>0$.
 As is customary (see, e.g.,~\cite{krause2014submodular}), instead of the  regret in Eq.~\eqref{eq:general_regret}, we consider the so-called $\alpha$-regret:
\begin{equation}
    \begin{split}
    \alpha\text{-}\mathrm{regret}_T ({\vec\P}_\X) \triangleq 
    \sup_{\parentheses{f_t}_{t=1}^{T}  \in {\F}^T} \bigg\{ \max_{\x\in \X}  \alpha\sum^T_{t=1} {f}_t(\x) 
     -\underset{{{\vec\P}_\X}}{\E} \interval{\sum^T_{t=1} {f}_t(\x_t)}\bigg\} 
    \label{eq:alpha_regret}.
    \end{split}
\end{equation}
 Intuitively, we compare the performance of the policy $\vec \P_{\X}$ w.r.t. the best {polytime}$(n)$ $\alpha$-approximation of the static offline optimum in hindsight. For example, the approximation ratio would be $\alpha=1-1/e$ in the case of submodular set functions maximized over matroids. %We define the $\alpha$-regret as
%As before, we seek policies that attain a sublinear (i.e., $o(T)$) $\alpha$-regret: such policies will perform on average as well as the best $\alpha$-approximation of the  static optimum in hindsight. 






\section{Online Submodular Optimization via Online Convex Optimization}
\label{sec:osmviaoco}

\subsection{The Case of General Set Functions}
\label{s:osm_genral}
\begin{algorithm}[t]

\caption{Rounding-Augmented OCO (RAOCO) policy}
\begin{algorithmic}[1]
\begin{footnotesize}
\Require OCO policy ${\vec\P}_{\Y}$, randomized rounding $\Xi:\Y \to \X$
% \Ensure $\aregret = o(T)$
\For {$t = 1,2,\dots, T$}
    \State $\y_t \gets \P_{\Y, t}\parentheses{ (\y_s)^{t-1}_{s=1}, (\cfunc_s)^{t-1}_{s=1}}$
\State $\x_t \gets \Xi (\y_t)$
\State Receive reward $f_t(\x_t)$
\State Reward function $f_t$  is revealed 
\State Construct $\cfunc_t$ from $f_t$ satisfying Asm.~\ref{assumption:sandwich}
\EndFor
\end{footnotesize}
\end{algorithmic}
\label{alg:saoco}
\end{algorithm}
First, we show how OCO can be leveraged to tackle online learning in the general combinatorial setting, i.e., when $\X\subseteq \{0,1\}^n$ and $\F$ comprises general  functions defined over $\X$. %In particular, we establish a formal property under which online learning in this setting can be reduced to OCO. %; in our next section, we show that this condition is indeed satisfied by online WTP maximization over matroid constraints.

\paragraph{Rounding Augmented OCO Policy.} 
We begin by stating a ``sandwich'' property that functions in $\F$ should satisfy, so that the reduction to OCO holds. To do so, we first need to introduce the notion of randomized rounding. Let  $\Y \triangleq \conv\X$ be the convex hull of $\X$. A \emph{randomized rounding}  is a random map ${\Xi:\Y \to \X}$, i.e., a map  from a fractional  $\y \in \Y$ and, possibly, a source of randomness to an integral variable $\x \in \X$.  We  assume that the set $\F$ satisfies the following:
\begin{assumption} (Sandwich Property)\label{assumption:sandwich}
There exists an $\alpha \in (0,1]$, an $L\in \reals_{>0}$, and a randomized rounding  $\Xi:\Y \to \X$ such that, for every $f : \X \to \reals_{\geq 0} \in \F$ there exists a $L$-Lipschitz concave function $\cfunc : \Y \to \reals$ s.t.   
\begin{align}
    \cfunc(\x) &\geq f(\x), \quad\text{for all $ \x \in \X$, and }\label{eq:alpha_approx_upper}
\end{align}
\vspace{-2em}
\begin{align}
    \E_{\Xi} \interval{f(\Xi(\y))} &\geq \alpha \cdot \cfunc(\y) ,\quad \text{ for all}~\y \in \Y. % and $\x = \Xi (\y)$ }.
    \label{eq:alpha_approx_lower}
\end{align}
%Moreover, function $\cfunc$ can be constructed from $f$ in polynomial time (in the representation of $f$).
\end{assumption}
We refer to $\cfunc$ as the \emph{concave relaxation} of $f$. Intuitively, Asm.~\ref{assumption:sandwich} postulates the existence of such a concave relaxation $\cfunc$ that is not ``far'' from $f$: Eqs.~\eqref{eq:alpha_approx_upper} and~\eqref{eq:alpha_approx_lower} imply that $\cfunc$ bounds $f$ both from above and below, up to the approximation factor $\alpha$. Moreover, the upper bound (Eq.~\eqref{eq:alpha_approx_upper}) needs to only hold for integral values, while the lower bound (Eq.~\eqref{eq:alpha_approx_lower}) needs to only hold in expectation, under an appropriately-defined randomized rounding $\Xi$. 

Armed with this assumption, we can convert any  OCO policy $\vec \P_\Y$ operating over  $\Y=\conv\X$ to a   \emph{Randomized-rounding Augmented OCO} (RAOCO) policy, denoted by $\vec\P_\X$, operating over $\X$. This transformation (see Alg.~\ref{alg:saoco}) uses both the randomized-rounding  $\Xi$, as well as the concave relaxations $(\cfunc_s)_{s=1}^{t-1}$ of the functions $(f_s)_{s=1}^{t-1}$ observed so far. %,  composed of an OCO policy $\vec \P_\Y$~\eqref{eq:onlineprotocol} operating over the convex set $\Y$ given by 
%\begin{align}
%    \Y \triangleq \conv\X;
%\end{align}
%And a randomized rounding scheme ${\Xi:\Y \to \X} $. 
%The rounding scheme $\Xi$ randomly rounds a fractional decision $\y \in \Y$ to an integral decision $\x \in \X$ for a given timeslot $t$, i.e., 
%\begin{align}
%    \P_{\X, t} &= \Xi \circ  \P_{\Y, t}.
%\end{align}
At $t \in \T$, the RAOCO policy amounts to:
\begin{subequations}
\label{eq:raoco}
\begin{align}
\y_t &=\P_{\Y, t}\parentheses{ (\y_s)^{t-1}_{s=1}, (\cfunc_s)^{t-1}_{s=1}}, \\
\x_t &=\Xi(\y_t)\in \X.
\end{align}
\end{subequations}
In short,  the OCO policy $\P_{\Y}$ is first  used to generate a new fractional state  $\y_t \in \Y$ by applying $\P_{\Y, t}$ to the  history of concave relaxations.
%is determined by an OCO policy that takes the history $({{(\y_s)}^{t-1}_{s=1} , {(\cfunc_s)}^{t-1}_{s=1}})$ (line~2 in Alg.~\ref{alg:saoco}), (2)
Then, this fractional decision $\y_t$ is randomly mapped to an integral decision $\x_t\in\X$ according to the rounding scheme $\Xi$. Then, the reward $f(\x_t)$ is received and $f_t$ is revealed, at which point a concave function $\cfunc_t$ is constructed from $f_t$ and added to the history. %The RAOCO policy in Eq.~\eqref{eq:raoco} can be thought of as $\P_{\X}=\Xi \circ \P_\Y$, i.e.,
%\begin{align}
%    \P_{\X, t}\parentheses{\parentheses{\x_s}^{t-1}_{s=1} , \parentheses{f_s}^{t-1}_{s=1}} &\triangleq \Xi \parentheses { \P_{\Y, t}\parentheses{(\y_s)^{t-1}_{s=1}, (\cfunc_s)^{t-1}_{s=1}} },
%\end{align}    
%    i.e., 
%it is the composition of the randomized rounding $\Xi$ with the OCO policy applied to $\Y$,  with rewards appropriately transformed. 
Our first main result is the following: %that, as a consequence of  Asm.~\ref{assumption:sandwich},  the RAOCO policy in Alg.~\ref{alg:saoco} attains the following $\alpha$-regret guarantee:
%\end{align}
 
 %We assume that the randomized rounding scheme $\Xi$ and the constructed functions $\cfunc_t$ satisfy the following assumption.
%
%\begin{assumption} (Sandwich Property)\label{assumption:sandwich}
%Consider $\alpha \in (0,1]$, for all $f : \X \to \reals_{\geq 0} \in %\F$ there exits a concave function $\cfunc : \Y \to \reals$ s.t. %$\cfunc$ satisfies Asm.~\ref{asm:oco} and 
%\begin{align}
%    \cfunc(\x) &\geq f(\x), & &\text{for $ \x \in %\X$}.\label{eq:alpha_approx_upper}
%\end{align}
%There exists a randomized rounding scheme $\Xi:\Y \to \X$ s.t.
%\begin{align}
%    \E_{\Xi} \interval{f(\x)} &\geq \alpha \cdot \cfunc(\y) , & & \text{ for $\y \in \Y$  and $\x = \Xi (\y)$ }.\label{eq:alpha_approx_lower}
%\end{align}
%\end{assumption}

 
\begin{theorem}
Under Asm.~\ref{assumption:sandwich}, given an OCO policy $\vec\P_\Y$,  the RAOCO policy $\vec\P_\X$ described by Alg.~\ref{alg:saoco} satisfies
%\begin{align}
   $ \aregret_T \parentheses{\vec\P_\X} \leq \alpha \cdot \regret_T \parentheses{{\vec{\P}}_{\Y}}.$
%\end{align}
\label{theorem:sandwich}
\end{theorem}
The proof is in \fullversion{Appendix~\ref{appendix:sandwich}}{Appendix~\ref{appendix:sandwich}}. As a result, \emph{any regret guarantee obtained by an OCO algorithm over $\Y$, immediately transfers to an $\alpha$-regret for RAOCO, where $\alpha$ is determined by Asm.~\ref{assumption:sandwich}.}
In particular, the decision set $\Y$ is closed, bounded, and convex by construction. Combined with the fact that concave relaxations $\cfunc$ are $L$-Lipschitz (by Asm.~\ref{assumption:sandwich}), Thms.~\ref{thm:oco} and~\ref{theorem:sandwich} yield the following  corollary:
\begin{corollary}\label{cor:raoco}
Under Asm.~\ref{assumption:sandwich},  RAOCO policy $\vec\P_\X$  in  Alg.~\ref{alg:saoco} equipped with OGA, OMA, or FTRL as OCO policy $\vec\P_\Y$  has sublinear $\alpha$-regret. That is, %\begin{align}
     $   \aregret_T\parentheses{\vec\P_\X} = \BigO{\sqrt{T}}.$
   % \end{align}
\end{corollary}
To make use of this result, we need Asm.~\ref{assumption:sandwich} to hold. We also need that both the randomized rounding and the concave relaxations used in RAOCO can be implemented in polynomial time. All of these statements are true for WTP functions optimized over matroid constraints, which we turn to next.

\subsection{The Case of Weighted Threshold Potentials} \label{s:osm_wtp}
We now consider the case where the decision set is a matroid, and reward functions belong to the class of WTP functions, defined by Eq.~\eqref{eq:wtp}. We will show that, under appropriate definitions of a randomized rounding and concave relaxations, the class $\F$ satisfies Asm.~\ref{assumption:sandwich} and, thus, online learning via RAOCO comes with the regret guarantees of Corollary~\ref{cor:raoco}.
%
Let again $\Y=\conv{\X}$ and consider the mapping $f\mapsto \cfunc$ of WTP functions $f:\X\to\reals$ to concave relaxations $\cfunc:\Y\to\reals$ of the form:
\begin{equation}
    \begin{split}
        \cfunc (\y) \triangleq f(\y) =\sum_{\ell \in C} c_{\ell} \min\set{b_\ell, \sum_{j \in S_\ell} y_j w_{\ell ,j}}, %\\
     %   \text{for $\y\in \Y$}.
     \label{eq:budget-additive-concave}
    \end{split}
\end{equation}
for $\y\in \Y$.  In other words, \emph{the relaxation of $f$ is itself}: it has the same functional form, allowing integral variables to become fractional.\footnote{In Appendix~\ref{appendix:alternate_relaxation}, we provide an example under which the concave relaxations do not share same functional form.} This is clearly concave, as the minimum of affine functions is concave, and the positively weighted sum of concave functions is concave. %This construction can be performed in polynomial time in the representation length of $f$. 
Finally, all such functions are Lipschitz, with a parameter that depends on $c_\ell$, $b_\ell$, $\vec w_\ell$, $\ell\in C$.
%
 Let $\cfuncSet$ be the image of $\F$ under the map \eqref{eq:budget-additive-concave}.
We make the following assumption, which is readily satisfied if, e.g., all constituent parameters ($c_\ell$, $b_\ell$, $\vec w_\ell$, $\ell\in C$) are uniformly bounded, or the set $\F$ is finite, etc.: 
\begin{assumption}\label{assumption:lip}
    There exists an $L>0$ such that all functions in $\cfuncSet$ are  $L$-Lipschitz.
\end{assumption}

%Consider a function in the class of WTP functions~\eqref{eq:wtp} $f: \set{0,1}^n \to \reals_{\geq 0}$ given as a weighted sum of  threshold potentials~\eqref{eq:budget-additive} 
%\begin{align}
%    f(\x) \triangleq \sum_{\ell \in C} c_{i} \Psi_{b_\ell,\vec w_\ell, S_\ell} (\x), \quad\text{for $\x \in \set{0,1}^n$}.
%\end{align}
%We define the concave function $\cfunc: \Y \to \reals_{\geq 0}$ as the extension of $f$ to the domain $\Y \triangleq {\conv{\X}}$, i.e., 
%\begin{align}ƒE
%    \cfunc (\y) \triangleq f(\y)  \quad \text{for $\y\in \Y$}.\label{eq:budget-additive-concave}
%\end{align}
%For each $i \in C$, the threshold potential $\Psi_{b_\ell,\vec w_\ell, S_\ell} (\y)$ is concave in $\y \in \Y$, because it is a composition of a concave function $\min \set{b_\ell, \,\cdot\,}$ and a linear term  $\sum_{j\in S_\ell} y_j w_{\ell,j}$. The function $\cfunc (\y)$ is concave in $\y \in \Y$ because it is a weighted sum with positive weights of concave functions in $\y \in\Y$.

Next, we turn our attention to the randomized rounding $\Xi$. We can in fact characterize the property that $\Xi$ must satisfy for Asm.~\ref{assumption:sandwich} to hold for relaxations given by Eq.~ \eqref{eq:budget-additive-concave}:
%We define the family of randomized rounding with \emph{negatively correlated} output as follows.
\begin{definition}
A randomized rounding  $\Xi:\Y \to \X$ is \emph{negatively correlated} if,  for $\x = \Xi(\y) \in \X$ (a) the coordinates of $\x$ are negatively correlated~\footnote{A set of random variables $x_i\in\set{0,1}, i \in [n]$, are  negatively correlated if  $\E\interval{\prod_{i \in S} x_i }\leq \prod_{i \in S} \E\interval{x_i}$ for all $S \subseteq [n]$.} %, and $\E\interval{\prod_{i \in S} (1-x_i) }\leq \prod_{i \in S} (1-\E\interval{x_i}).$} 
and (b)  $\E_\Xi\interval{\x} = \y$.\label{def:negatively_correlated_sampler}
\end{definition}
%Under this setting, we identify the randomized rounding scheme and the concave functions $\cfunc$  that satisfy the requirements in Asm.~\ref{assumption:sandwich}. Formally, we have:
Our next result immediately implies that \emph{any negatively correlated rounding can be used in RAOCO}: 
\begin{lemma}\label{proposition:sandwich2}
Let $\Xi:{\Y} \to \X$ be a negatively correlated randomized rounding, and consider the concave relaxations $\cfunc$ constructed from $f\in\F$ via Eq.~\eqref{eq:budget-additive-concave}. Then, if Asm.~\ref{assumption:lip} holds for some $L>0$, the set $\F$ satisfies Asm.~\ref{assumption:sandwich} with 
 $\alpha = \parentheses{1 - \frac{1}{\Delta}}^\Delta$ where $\Delta = \sup_{f\in \F}\Delta_f$.%, a negatively correlated randomized rounding scheme $\Xi:{\Y} \to \X$ (Def.~\ref{def:negatively_correlated_sampler}), and functions $f: {\Y} \to \reals_{\geq 0}$ and $\cfunc:\X \to \reals_{\geq 0}$ in Eqs.~\eqref{eq:budget-additive} and \eqref{eq:budget-additive-concave}, respectively. Then  Asm.~\ref{assumption:sandwich} is satisfied.
\end{lemma}
The proof is in \fullversion{Appendix~\ref{appendix:sandwich2}}{Appendix~\ref{appendix:sandwich2}}. As $\Delta\to\infty$, the approximation ratio $\alpha$ approaches $1-1/e$ from above, recovering the usual approximation guarantee. However, for finite $\Delta$, we in fact obtain an improved approximation ratio; an example (quadratic submodular functions) is described in \fullversion{Appendix~\ref{appendix:WTP}}{Appendix~\ref{appendix:WTP}}. 
%
%We conclude from Theorem~\ref{theorem:sandwich}  that an $\alpha$-regret guarantee is attained under this setting. We obtain the following corollary:
% \begin{corollary}
%     Under weighted threshold potentials rewards in Eq.~\eqref{eq:budget-additive}  and concave functions in Eq.~\eqref{eq:budget-additive-concave},  RAOCO policy in Alg.~\ref{alg:saoco} $\vec\P_\X$ equipped with an OMA policy in  Alg.~\ref{alg:oma} configured with negative entropy $\Phi = \sum_{i \in V} x_i \log(x_i) $ satisfying Asms.~\ref{asm:mirror_map}--\ref{asm:bounded_gradient_mirror_map} 
%  and a fixed learning rate $\eta = $ has sublinear $\alpha$-regret, i.e.,
%     \begin{align}
          % \aregret\parentheses{\vec\P_\X} = \alpha  \max\set{\sum_{\substack{i \in C, k \in S_i}}  w_i: k \in V} \sqrt{2 r^2_\X\log\parentheses{\frac{n}{r_\X}} T}.
    % \end{align}
    % % where $r_\X = \max_{\x \in \X} \norm{\x}_1$.
% \end{corollary}
%
%
%
% Note that Asm.~\ref{asm:oco} is attained from the definition of the threshold functions~\eqref{eq:budget-additive} and the supergradients expression in Eq.~\eqref{eq:subgradient}. The $\norm{\,\cdot\,}_\infty$-norm of supergradients is bounded by $L\triangleq\max\set{\sum_{\substack{i \in C\\k \in S_i}}  w_i: k \in V}$, i.e., $\cfunc$ is $L$-Lipschitz w.r.t. the $\norm{\,\cdot\,}_1$ norm.  Thus, RAOCO policy in Alg.~\ref{alg:saoco} $\vec\P_\X$ equipped with an OCO policy (e.g., OGD and OMD) has sublinear $\alpha$-regret, i.e., $\aregret\parentheses{\vec\P_\X} = \BigO{\sqrt{T}}$.
%
% \subsubsection{Characterization of the Sampler} 
%
Finally, and most importantly, \emph{a negatively-correlated randomized rounding  can always be constructed if $\X$ is  matroid}. This construction is classic:~\citet{chekuri2010dependent} provide two polynomial-time randomized rounding algorithms that satisfy this property: 
\begin{lemma} (\citet[Theorem~1.1.]{chekuri2010dependent})\label{theorem:rounding}
    Given a matroid $\X\subset\{0,1\}^n$, let $\y \in \conv{\X}$  and $\Xi$ be either  \emph{swap rounding} or \emph{randomized pipage rounding}. Then, $\Xi$ is negatively correlated.
\end{lemma}
We review swap rounding, for completeness, in \fullversion{Appendix~\ref{appendix:swap}}{Appendix.~\ref{appendix:swap}}. Interestingly,~\citet{chekuri2010dependent} prove that the existence of a negatively correlated rounding is inherently linked to  matroids: a negatively-correlated rounding exists \emph{if and only if~$\X$ is a matroid} (see Thm.~I.1. in \cite{chekuri2010dependent}). Our Lemma~\ref{proposition:sandwich2} thus implies that the reduction of RAOCO to OCO policies is also closely linked to matroid constraints.
%
Putting everything together, Lemmas~\ref{proposition:sandwich2}--\ref{theorem:rounding} and Corollary~\ref{cor:raoco} yield the following theorem:
\begin{theorem}\label{thm:main2}
Let $\X\subseteq\{0,1\}^n$ be a matroid, and  $\F$ be a subset of the WTP class for which Asm.~\ref{assumption:lip} holds. Then, the RAOCO policy $\vec \P_\X$ defined by Alg.~\ref{alg:saoco} using swap rounding or randomized pipage rounding as $\Xi$ and OGA, OMA, or FTRL as OCO policy $\vec\P_\Y$, and  concave relaxations in Eq.~\eqref{eq:budget-additive-concave}  
 has sublinear $\alpha$-regret. In particular, %\begin{align}
     $   \aregret\parentheses{\vec\P_\X} = \BigO{\sqrt{T}}.$
\end{theorem}
Note that, though all algorithms yield $O(\sqrt{T})$ regret, the dependence of constants on problem parameters (such as $n$ and the matroid rank $r$), as reported in Table~\ref{table:compare}, is optimized under OMA (see Appendix~\ref{appendix:setups_omd}). 

\subsection{Computational Complexity}
%We conclude our analysis with the time complexity of Alg.~\ref{alg:saoco}.% in the general WTP setting; we discuss specific examples in Sec.~\ref{sec:examples}.

\paragraph{OCO Policy.} OCO policies are polytime, and their analysis is classic (see, e.g.,~\cite{hazan2016introduction}). Taking gradient-based OCO policies (e.g., OMA in {Alg.~\ref{alg:oma}} of the supplement), their computational complexity is  dominated by a projection operation to the convex set $\Y=\conv\X$. %This is most expensive operation computationally since the gradient update step is linear-time $\BigO{n}$. 
The exact time complexity of this projection depends on  $\Y$, however, given a membership oracle that decides $\y \in \conv\X$, the projection can be computed efficiently in polynomial time~\cite{hazan2016introduction}. Moreover, the projection problem is a convex problem that can be computed efficiently (e.g., iteratively to an arbitrary precision) and can also be computed in strongly polynomial time~\cite[Theorem~3]{gupta2016solving}.%#

\input{figs/experimental_result_table}

\paragraph{Concave Relaxations and Randomized Rounding.}  Concave relaxations are linear in the representation of the function $f$, but in practice come ``for free'', once parameters in Eq.~\eqref{eq:wtp} are provided.   Swap rounding over a general matroid is  $\BigO{n r^2}$, where %$n$ is the size of the ground set and 
$r$ is the rank of the matroid~\cite{chekuri2010dependent}. This dominates the remaining operations (including OCO), and thus determines the overall complexity of our algorithm.
This $\BigO{n r^2}$ term assumes access to decomposition of a fractional point $\y \in \Y$ to bases of the matroid. Carathéodory's theorem implies the existence of such decomposition of at most $n+1$ points in $\X$; moreover, there exists a decomposition algorithm~\cite{cunningham1984testing} for general matroids with running time $\BigO{n^6}$. 
However, in all practical cases we consider (including uniform and partition matroids) the complexity is significantly lower. More specifically,
for partition matroids,  swap rounding reduces to an algorithm with linear time complexity, namely, $\BigO{m n}$ for $m$ partitions~\cite{Srinivasan2001}. %The procedure takes a fractional $\y = (y_1, y_2, ..., y_n) \in [0, 1]^n$ satisfying the cardinality constraint $\sum_{i=1}^{n} y_i = r \in \naturals$. Then, it rounds $\y$ into an integral $\x = (x_1, x_2, ... x_n) \in \{0, 1\}^n$. The algorithm is as follows. Until all $x_i$'s are fixed to either $0$ or $1$ repeat the following. Select two unfixed variables $x_i$ and $x_j$ and call a subroutine  that fixes randomly at least one variable in $\BigO{1}$ steps. Therefore, for each cardinality constraint in the partition matroid the  rounding procedure completes in $\BigO{n}$ steps, and this yields a total $\BigO{mn}$ time complexity.



%\paragraph{Construction of Concave Rewards.} Construction of concave rewards under threshold potentials~\ref{eq:budget-additive} comes for free. Because the functions can be constructed by  extending the value of $f$ over fractional values in $[0,1]^n$.

%\paragraph{Oracles and Overall Complexity.} We characterize the overall complexity of our policy assuming access to a projection oracle and a decomposition oracle, because time complexity of the projection and decomposition of $\x$ to a convex combination of points in $\X$ heavily depends on the particular structure of $\conv\X$. Hence, under such a construction, the most expensive operation is the randomized rounding scheme that can be performed in $\BigO{n^2 r}$.





\section{Extensions}\label{sec:extensions}

\paragraph{Dynamic Setting.} In the dynamic setting, the decision maker compares its performance to the best sequence of decisions $(\y^\star_t)_{t \in \T} $ with a path length {regularity} condition~\cite{zinkevich2003,cesa2012mirror}. I.e., let
$\Lambda_{\X} (T,P_T) \triangleq \set{\parentheses{\x_t}^T_{t=1} \in \X^T: \sum^T_{t=1} \norm{\x_{t+1} - \x_t} \leq P_T} \subset \X^T$
be the set of sequences of decision in a set $\X$ with path length less than $P_T \in \reals_{\geq 0}$ over a time horizon $T$. We extend the definition of the regret (Eq.~\eqref{eq:alpha_regret}) to that of  \emph{dynamic $\alpha$-regret}: 
\begin{align*}
     &\alpha\text{-}\mathrm{regret}_{T, P_T} ({\vec\P}_\X) \triangleq  \sup_{\parentheses{{f}_t}^T_{t=1} \in {\F}^T} \bigg\{\max_{\parentheses{\x^\star_t}^T_{t=1}\in    \Lambda_{\X} (T,P_T)}  \alpha\sum^T_{t=1} {f}_t(\x^\star_t) -\sum^T_{t=1} {f}_t(\x_t)\bigg\} %\label{eq:dynamic_alpha_regret}.
\end{align*}
When $\alpha\text{-}\mathrm{regret}_{T, P_T}({\vec\P}_\X)$  is sublinear in $T$, the policy attains average rewards that asymptotically compete with the optimal decisions \emph{of bounded path length}, in hindsight.


Through our reduction to OCO, we can  leverage  OGA \cite{zinkevich2003} or meta-learning algorithms over OGA~\cite{zhao2020dynamic} to obtain dynamic regret guarantees in OSM. As an additional technical contribution, we provide  the first sufficient and necessary conditions for OMA to admit a dynamic regret guarantee (see Appendix~\ref{appendix:oco}). This allows to extend a specific instance of OMA operating on the simplex,  the so-called fixed-share algorithm~\cite{cesa2012mirror,herbster1998tracking},  to  matroid polytopes.  This yields a tighter regret guarantee than OGA~\cite{zinkevich2003,zhao2020dynamic} (see Theorem~\ref{thm:general_regret_dynamic+optimistic} in Appendix~\ref{appendix:oco}).
Putting everything together,  we get:
\begin{theorem}\label{thm:dynamic}
Under Asm.~\ref{assumption:sandwich},  RAOCO policy $\vec\P_\X$  described by  Alg.~\ref{alg:saoco} equipped with  an OMA policy in Appendix~\ref{appendix:oco} as OCO policy $\vec\P_{\Y}$ 
    % When the concave functions $\cfunc$ in Asm.~\ref{assumption:sandwich} satisfy Asm.~\ref{asm:oco}, then  RAOCO policy in Alg.~\ref{alg:saoco} $\vec\P_\X$ equipped with an OMA policy in \fullversion{Supplementary Material}{Alg.~\ref{alg:oma}} configured with $\Phi$ satisfying Asms.~\fullversion{\textcolor{red}{\textbf{(?)--(?)}} in the supplement}{\ref{asm:mirror_map}--\ref{asm:bounded_gradient_mirror_map}} 
 % and a fixed learning rate $\eta_\star  = \sqrt{\frac{2\rho \parentheses{D^2 + 2 L_\Phi P_T}}{L^2 T}}$ 
 has sublinear dynamic $\alpha$-regret, i.e.,     
 %\begin{align}
 $    \alpha\text{-}\mathrm{regret}_{T,P_T} ({\vec\P}_\X) = \BigO{\sqrt{P_T T} }.$
   % \end{align}
\end{theorem}
This follows from Thm.~\ref{theorem:sandwich} and the dynamic regret guarantee for OMA    we establish  in Appendix~\ref{appendix:oco}.






\paragraph{Optimistic Setting.} 
\label{s:optimism}
In the optimistic setting, the decision maker has access to additional information available in the form of predictions: a  function $\pi_{t+1}:\interval{0,1}^n \to \reals_{\geq 0}$,  serving as a prediction of the reward function $f_{t+1}(\x)$ is made available  before committing to a decision $\x_{t+1}$ at timeslot $t \in \T$.  The prediction $\pi_t$  encodes prior information available to the decision maker at timeslot $t$.\footnote{Function $\pi_t$ can extend over fractional values, e.g.,  be the multi-linear relaxation of a set function.}  Let  $\g_t$ and $\pg_t$ be supergradients of $\cfunc_t$ and $\pi_t$ at point $\y_t$, respectively.  We can define an optimistic OMA policy 
(see Alg.~\ref{alg:ooma}  in Appendix~\ref{appendix:oco}) that leverages both the prediction and the observed rewards. Applying again our reduction of OSM to this setting we get:
\begin{theorem}\label{thm:osm_optimistic}
Under Asm.~\ref{assumption:sandwich},  RAOCO policy $\vec\P_\X$  in Alg.~\ref{alg:saoco} equipped with  OOMA in Appendix~\ref{appendix:oco} as policy $\vec\P_{\Y}$ yields
    % \begin{align}
  $   \alpha\text{-}\mathrm{regret}_{T, P_T} ({\vec\P}_\X)=\BigO{P_T \sqrt{\sum^T_{t=1}\norm{\g_t - \pg_t}^2_\infty}}.$ %\end{align}
\end{theorem}
This theorem follows from Theorem~\ref{theorem:sandwich} and the optimistic regret guarantee established for OMA policies in Theorem~\ref{thm:general_regret_dynamic+optimistic} in Appendix~\ref{appendix:oco}.
%
The optimistic regret guarantee in Theorem~\ref{thm:osm_optimistic} shows that the regret of a policy can be reduced to $0$ when the predictions are perfect, while providing $\BigO{\sqrt{T}}$ guarantee in Thm.~\ref{thm:main2} when the predictions are arbitrarily bad (with bounded gradients).
To the best of our knowledge, ours is the first work to provide guarantees for  optimistic OSM.



\paragraph{Bandit Setting.}
\label{s:bandit}
Recall that in the bandit setting the decision maker  only has  access to the reward $f_t(\x_t)$ after committing to a decision $\x_t \in \X$ at $t\in\T$; i.e., the reward function is \emph{not} revealed. 
Our reduction to OCO does not readily apply to the bandit setting; however, we show that the bandit algorithm by \citet{wan2023bandit} can be used to construct such a reduction. The main challenge is to estimate gradients of inputs in $\Y$ only from bandit feedback; this can be done via a perturbation method (see also~\citet{hazan2014bandit}). This approach, described in Appendix~\ref{appendix:extensions}, yields the following theorem:
%Our algorithm for regret-minimization in this setting is given in 
%Appendix~\ref{appendix:extensions}.  In this setting, a policy does not have access to the full supergradients due to the bandit feedback. However, estimates of supergradients can be constructed by perturbing around points in $\Y$~\cite{hazan2014bandit}. We construct a policy that explores through perturbations and exploits through an OCO policy. 
 % A challenge arises because the perturbations should not yield points outside this $\Y \triangleq \conv\X$ ; otherwise, we may not be able to apply the randomized rounding scheme $\Xi$ on perturbed points in Asm.~\ref{assumption:sandwich}, which is tied to $\Y$.  When $\Y$ contains  a unit ball centered around $\vec 0$; such a set can easily be constructed through a simple rescaling~\cite{hazan2014bandit}; however, in our setting, this  does not hold. We show that when $\Y$ is determined by a matroid polytope,  we can construct a translation of this set  such that the resulting set $\Y_\delta$ is  convex and contained in $\Y$; moreover,  perturbations of  points in $\Y_\delta$ by $\delta$  are always contained in $\Y$. We define this set $\Y_\delta$ for $\delta \in (0, 1/2n]$ as the range of an affine mapping $T:\Y \to \Y_\delta$ where $ T(\y) = (1 - 2n \delta)  \y  + \delta \vec 1$ for every point  $\y$ in $\Y$, i.e.,  $ Y_\delta \triangleq \set{ T(\y): \y\in \Y}$.  
 
\input{figs/plots} 
 
\begin{theorem} Under bounded submodular monotone rewards and partition matroid constraint sets, LIRAOCO policy $\vec\P_\X$  in Alg.~\ref{alg:lisaoco} in Appendix~\ref{appendix:extensions} equipped with  an OCO policy $\vec\P_{\Y_\delta}$  \label{theorem:bandit}
yields 
 $   \aregret_{T, P_T, W} \parentheses{\vec\P_\X} \leq  W \cdot \mathrm{regret}_{T/W, P_T} \parentheses{\vec{\P}_{\Y_\delta}} + \frac{T}{W} + 2 \alpha \delta r^2 n   T,$
 where $\delta, W$, are tuneable parameters of the algorithm and  $\mathrm{regret}_{T/W, P_T} \parentheses{\vec{\P}_{\Y_\delta}}$ is the regret of an OCO policy executed for $T/W$ timeslots.
\end{theorem}
%The proof of this theorem is  in Appendix~\ref{appendix:extensions}. 
We note that this result applies to general submodular functions, but is restricted to partition matroids.  We also note that this also extends to dynamic  and optimistic settings: we provide the full description in  Appendix~\ref{appendix:extensions}. Our analysis generalizes  \citet{wan2023bandit} in that (a) we show that a reduction can be performed to any OCO algorithm, rather than just FTRL, as well as  (b) in extending it to the dynamic and optimistic settings %. However, the regret attained through the reduction to an arbitrary OCO algorithm  ($\aregret \parentheses{\vec\P_\X}  = \BigO{T^{4/5}}$) is higher than with the specific instance of FTRL used by~\citet{wan2023bandit} ($\BigO{T^{2/3}}$), which however does not extend to the dynamic and optimistic settings 
(see also Table~\ref{table:compare2} in the appendix).
%Note that under appropriate configurations of the different parameters $ W, \delta$ and OCO policy $\P_{\Y_\delta}$, the regret attained is $\aregret \parentheses{\vec\P_\X}  = \BigO{T^{4/5}}$. This rate can further be improved to $\aregret \parentheses{\vec\P_\X}  = \BigO{T^{3/2}}$ under static regret by configuring LIRAOCO with  $\delta = 0$   and OCO policy FTRL in Alg.~\ref{alg:ftrl} in Appendix~\ref{appendix:oco} configured with a self-concordant barrier regularizer. 







\section{Experiments}\label{sec:experiments}

\paragraph{Datasets and Problem Instances.} We consider five different OSM problems: two are influence maximization problems, over the \IMZKC{} \cite{zachary1977information} and \IMEpinions{} 
\cite{epinions} graphs, respectively, a facility location problem over the \FLMovieLens{} dataset \cite{movielens}, a team formation and a weighted coverage problem over synthetic datasets. Reward functions are generated over a finite horizon and optimized online over both uniform and partition matroid constraints. 
The five settings are summarized in Table~\ref{tab:exp} in the Appendix; additional details for each dataset and setting are provided in Appendix~\ref{appendix:experiments}.


\paragraph{Algorithms.} We implement the policy in Alg.~\ref{alg:saoco} (\Algorithm{RAOCO}), coupled with \Algorithm{OGA} (\RAOCOOGA{}) and \Algorithm{OMA} (\RAOCOOMA{}) as OCO policies. As competitors, we also implement the \emph{fixed share forecaster} (\Algorithm{FSF$^\star$}) policy by~\citet{matsuoka2021tracking}, which only applies to uniform matroids, and the 
\Algorithm{TabularGreedy} policy by~\citet{onlineassignement}, as well as a \Algorithm{Random} algorithm, which selects a decision u.a.r.~from the bases of $\X$.
We explore several hyperparameters for these policies; %, such as the learning rate $\eta$, $\gamma$, and number of experts $c_{\mathrm p}$; 
a full description of this exploration and additional details are reported in Appendix~\ref{appendix:experiments}.
% We will make our code  publicly available. %Should I point out that our results are fully reproducible?

\paragraph{Metrics.} For each setting, we compute $F^\star = \max_{\y\in \Y}\frac{1}{T}\sum_{t=1}^T\cfunc(\y)$, the value of the optimal fractional solution in hindsight, assuming rewards are replaced by their concave relaxations. 
Note that this involves solving a convex optimization problem, and overestimates the (intractable) offline optimal, i.e., $F^\star\geq \max_{\x\in \X}\frac{1}{T}\sum_{t=1}^Tf(\x)$. 
For each online policy, we compute both the integral and fractional average cumulative reward at different timeslots $t$, given by $\bar{F}_{\X} =\frac{1}{t}\sum_{s=1}^tf(\x_s)$,  $\bar{F}_{\Y} =\frac{1}{t}\sum_{s=1}^t\cfunc(\y_s)$, respectively.
We repeat each experiment for $5$ different random seeds, and use this to report standard deviations.


%We execute Alg.~\ref{alg:saoco} (\Algorithm{RAOCO}) over weighted coverage and quadratic set function instances using both real and synthetic datasets and compare its performance to the algorithm described by \cite{kakade2007playing}, which we refer to as the \Algorithm{KKL} algorithm. As a baseline we have also implemented a Random algorithm (\Algorithm{RA}) that selects a random decision at every iteration. We summarize the datasets and the variables we use in Tab.~\ref{tab:exp}. Our code will be publicly accessible after the revision.

\paragraph{OSM Policy Comparison.} A comparison between the two different versions of \Algorithm{RAOCO} (\Algorithm{OGA} and \Algorithm{OMA}) with the three competitors is shown in Table~\ref{tab:res}. We also report running time per timeslot as well as $\bar{F}_\Y$ in the supplement.  We observe that both \Algorithm{OGA} and \Algorithm{OMA} significantly outperform competitors, with the exception of \texttt{MovieLens}, where \Algorithm{TabularGreedy} does better. \Algorithm{OMA} is almost always better than \Algorithm{OGA}. Most importantly, we significantly outperform both \Algorithm{TabularGreedy} and \Algorithm{FSF$^\star$} w.r.t.~running time, being $2.15-250$ times faster (see Appendix~\ref{appendix:experiments}).

\paragraph{Dynamic Regret and  Optimistic Learning.} Fig.~\ref{fig:dynamicregret} shows the performance of the different policies in a dynamic scenario. All the policies have similar performance in the stationary setting, however in the non-stationary setting only \Algorithm{OGA}, \Algorithm{OMA}, and \Algorithm{FSF$^\star$} show robustness. We further experiment with an optimistic setting in Fig.~\ref{fig:optimistic_figure} under a non-stationary setting where we provide additional information about future rewards to the optimistic policies, which can leverage this information and yield better results  (see Appendix~\ref{appendix:experiments}).


\section{Conclusion}
\label{sec:conclusions}
We provide a reduction of  online maximization of a large class of submodular
functions  to online convex optimization and  show that our reduction extends to many different versions of the online learning problem.
There are many possible extensions. As our framework does not directly apply to general submodular functions, it would be interesting to derive a  general method to construct the concave relaxations which are the building block of our reduction in Sec.~\ref{s:osm_genral}. It is also meaningful to investigate the applicability of our reduction to monotone submodular functions with bounded curvature~\cite{feldman2021guess}, and non-monotone submodular functions~\cite{krause2014submodular}.





%\subsection{Algorithms}

%\paragraph{RAOCO.} We explore the following policies: 
%Online Gradient Ascent (\RAOCOOGA{}) and Online Mirror Ascent (\RAOCOOMA{}).
%\paragraph{other}
%\paragraph{other}
%\paragraph{Random Algorithm} As a baseline we implement a Random Algorithm (\Algorithm{RA}) playing a random decision at %each iteration.


%\subsection{Experimental Setup}
%(+Environment in which we run the experiments)


%\paragraph{Dynamic and Online Regret} \si{XXXX....}
% \begin{figure}[h]
% \centering
% \subfigure[\texttt{ZKC}, k=1]{
% \begin{minipage}{0.30\textwidth}
% \centering
% \includegraphics[width=1\textwidth]{figs/ZKC_100_01_k_1_100_iter_rewards.pdf}
% \centering
% \label{fig:ZKC1}
% \end{minipage}
% }
% \subfigure[\texttt{ZKC}, k=2]{
% \begin{minipage}{0.30\textwidth}
% \centering
% \includegraphics[width=1\textwidth]{figs/ZKC_100_01_k_2_100_iter_rewards.pdf}
% \centering
% \label{fig:ZKC2}
% \end{minipage}
% }
% \subfigure[\texttt{ZKC}, k=3]{
% \begin{minipage}{0.30\textwidth}
% \centering
% \includegraphics[width=1\textwidth]{figs/ZKC_100_01_k_3_100_iter_rewards.pdf}
% \centering
% \label{fig:ZKC3}
% \end{minipage}
% }
% \subfigure[\texttt{ZKC}, k=4]{
% \begin{minipage}{0.30\textwidth}
% \centering
% \includegraphics[width=1\textwidth]{figs/ZKC_100_01_k_4_100_iter_rewards.pdf}
% \centering
% \label{fig:ZKC4}
% \end{minipage}
% }
% \subfigure[\texttt{ZKC}, k=5]{
% \begin{minipage}{0.30\textwidth}
% \centering
% \includegraphics[width=1\textwidth]{figs/ZKC_100_01_k_5_100_iter_rewards.pdf}
% \centering
% \label{fig:ZKC5}
% \end{minipage}
% }
% \caption{Trajectory of the OGD algorithm. Cumulative averaged rewards are plotted.} 
% \label{fig:CGiters}
% \end{figure}


